CobBO: Coordinate Backoff Bayesian Optimization with Two-Stage Kernels

Bayesian optimization is a popular method for optimizing expensive black-box functions. Yet it oftentimes struggles in high dimensions where the computation could be prohibitively heavy. To alleviate this problem, we introduce Coordinate backoff Bayesian Optimization (CobBO) with two-stage kernels. During each round, the first stage uses a simple coarse kernel that sacrifices the approximation accuracy for computational efficiency. It captures the global landscape by purposely smoothing away local fluctuations. Then, in the second stage of the same round, past observed points in the full space are projected to the selected subspace to form virtual points. These virtual points, along with the means and variances of their unknown function values estimated using the simple kernel of the first stage, are fitted to a more sophisticated kernel model in the second stage. Within the selected low dimensional subspace, the computational cost of conducting Bayesian optimization therein becomes affordable. To further enhance the performance, a sequence of consecutive observations in the same subspace are collected, which can effectively refine the approximation of the function. This refinement lasts until a stopping rule is met determining when to back off from a certain subspace and switch to another. This decoupling significantly reduces the computational burden in high dimensions, which fully leverages the observations in the whole space rather than only relying on observations in each coordinate subspace. Extensive evaluations show that CobBO finds solutions comparable to or better than other state-of-the-art methods for dimensions ranging from tens to hundreds, while reducing both the trial complexity and computational costs.

==> abstract/abstract_v1.tex <==
\begin{abstract}
Coordinate backoff Bayesian optimization (CobBO) is designed to reduce trial complexity for optimizing black-box functions in both low and high dimensions. 
The principle is to capture the global landscape of the objective function by smoothed interpolations in randomly selected coordinate subspaces. Based on the already queried points, each iteration constructs a new set of virtual points projected on a random subspace. These virtual points, together with their interpolated function values, serve as the conditional events for computing the posterior distributions.  
This method can be viewed as a variant of coordinate ascent, tailored to Bayesian optimization using a backoff stopping rule. This stopping rule determines the number of consistent queries within each selected subspace before backing off.
Jointly, the random projection, the interpolation and the Gaussian regression yield a composite random kernel. This approach shows great promise in searching for the optimal solution in both low and high dimensions.
As a holistic framework, it also integrates data filtering by using selected points to accelerate computation and forms trust regions to encourage exploitation.
Through comprehensive evaluations on a wide spectrum of benchmarks, we show that CobBO can consistently find comparable or better solutions using the default setting, with reduced trial complexity compared to the state-of-the-art methods. 
\end{abstract}

==> abstract/abstract_v2.tex <==
\begin{abstract}
Bayesian optimization is a popular optimization method for expensive black-box functions. 
When based on Gaussian process regression for high-dimensional problems, this method requires many observations for a sufficient estimation of the objective function's landscape.
As hard real world problems of those characteristics require several thousands observations, the associated computational costs make the application of Bayesian optimization challenging, and often noncompetitive with other paradigms or even unpractical. 
We introduce Coordinate Backoff Bayesian optimization (CobBO) to alleviate those challenges. 
The high dimensionality is tackled by randomly selecting promising sets of coordinates thus effectively lower dimensional subspaces are explored, 
while leveraging full dimensional queried points through projection and smooth function interpolations. 
This approach can be viewed as a variant of coordinate ascent, tailored for Bayesian optimization using a stopping rule for backing off from a certain subspace and switching to another. %coordinate set.
Besides implicitly reducing the required observations due to the lower dimensional subspaces involved, 
aiming for a holistic practical method, 
CobBO is further accelerated by forming trust regions and discarding far from boundary or clustered data points.
% , with the added value of improved statistics and encouraging exploitation within promising local regions and filtering out local fluctuations of the objective function.
Through comprehensive evaluations on a wide spectrum of benchmarks, CobBO is shown to consistently find comparable or better solutions, with a reduced trial complexity compared to the state-of-the-art methods in both low and high dimensions.
\end{abstract}

==> abstract/abstract_v3.tex <==
\begin{abstract}
Bayesian optimization is a popular method for optimizing expensive black-box functions. 
The objective functions of hard real world 
problems are oftentimes characterized by a fluctuated landscape of many local optima. 
Bayesian optimization risks in over-exploiting such traps, remaining with insufficient query budget for exploring the global landscape.
%especially in high dimensions, where more observations are required for its efficient estimation.\\
We introduce Coordinate Backoff Bayesian optimization (CobBO) to alleviate those challenges. 
%For avoiding local optima, 
CobBO captures a smooth approximation of the global landscape by interpolating the values of queried points projected to randomly selected promising subspaces. Thus also a smaller query budget
%for exploration 
is required for the Gaussian process regressions applied over the lower dimensional subspaces. 
This approach can be viewed as a variant of coordinate ascent, tailored for Bayesian optimization, using a stopping rule for backing off from a certain subspace and switching to another coordinate subset. 
%Additionally, adaptive trust regions are dynamically formed to %expedite the convergence, and stagnant local optima are %escaped by switching trust regions.
%Further smoothness and acceleration are achieved by filtering %out clustered queried points. 
%and stagnant local optima are escaped by alternating between adaptive trust regions.\\
Extensive evaluations show that CobBO finds solutions comparable to or better than other state-of-the-art methods for dimensions ranging from tens to hundreds, while reducing the trial complexity.
%both low and high dimensions.
\end{abstract}

==> abstract/abstract_v4.tex <==
\begin{abstract}
Bayesian optimization is a popular method that oftentimes suffers from high dimensions. % for optimizing expensive black-box functions. 
%The objective functions of hard real world 
%problems are oftentimes characterized by a fluctuated landscape of many local optima. 
%Bayesian optimization risks in over-exploiting such traps, remaining with insufficient query budget for exploring the global landscape.
%especially in high dimensions, where more observations are required for its efficient estimation.\\
We introduce Coordinate backoff Bayesian optimization (CobBO) with two-stage kernels to alleviate this problem.
%due to curse of dimensionality. 
In each iteration, the first stage in the full space adopts a simple kernel that sacrifices the approximation accuracy in high dimensions
%for the sake of 
for computational efficiency. It captures a smooth approximation of the global landscape by interpolating the values of queried points projected to selected promising subspaces. 
%Thus also a smaller query budget
%is required for the Gaussian process regressions applied over the lower dimensional subspaces. 
The second stage of the same iteration in a selected coordinate subspace applies a sophisticated kernel that can tolerate high computational cost in low dimensions. It refines the approximation of the local landscape by a sequence of observations determined by a stopping rule to back off from a certain subspace and switch to another coordinate subset. 
%While the coordinate subspace selection makes CobBO efficient
%in each coordinate subspace, to avoid 
%in high dimensions, 
The two-stage kernel Gaussian process regressions fully leverage the observations in the whole space rather than only relying on observations in each coordinate subspace.
% restricts the attention on a subspace by thus also a smaller query budget.  
%The two-stage composite kernels decouple the Gaussian process regression and the acquisition maximization. 
%This decoupling 
%Together with the stopping rule, CobBO
This decoupling significantly reduces the computation time in high dimensions.
%This approach can be viewed as a variant of coordinate ascent, tailored for Bayesian optimization, using a stopping rule for backing off from a certain subspace and switching to another coordinate subset. 
More importantly, extensive evaluations show that CobBO finds solutions comparable to or better than other state-of-the-art methods for dimensions ranging from tens to hundreds, while reducing the trial complexity.
%both low and high dimensions.
\end{abstract}

==> abstract/abstract_v5.tex <==
\begin{abstract}
Bayesian optimization is a popular method for optimizing expensive black-box functions.
%
Yet it oftentimes struggles in high dimensions where the computation could be prohibitively expensive and a sufficient estimation of the global landscape requires more observations.
We introduce Coordinate backoff Bayesian optimization (CobBO) with two-stage kernels to alleviate this problem.  
In each iteration, a promising subset of coordinates is selected in the first stage, as past observed points in the full space are projected to the selected subspace adopting a simple kernel that sacrifices the approximation accuracy for computational efficiency.
Then in the second stage of the same iteration a more sophisticated kernel is applied for estimating the landscape in the selected low dimensional subspace where the computational cost becomes affordable. 
Effectively, this second stage refines the approximation of the global landscape estimated by the first stage through a sequence of observations in the same local subspace. This refinement lasts until a stopping rule is met determining when to back off from a certain subspace and switch to another coordinate subset. 
This decoupling significantly reduces the computational burden in high dimensions, while the two-stage kernels of the Gaussian process regressions fully leverage the observations in the whole space rather than only relying on observations in each coordinate subspace.
Extensive evaluations show that CobBO finds solutions comparable to or better than other state-of-the-art methods for dimensions ranging from tens to hundreds, while reducing the trial complexity and computational costs.
\end{abstract}



\begin{abstract}
Bayesian optimization is a popular method for optimizing expensive black-box functions. 
%
Yet it oftentimes struggles in high dimensions where the computation could be prohibitively heavy. 
While a complex kernel with many length scales are prone to overfitting and expensive to train, a simple kernel with too few length scales cannot effectively capture the variations of the high dimensional function in different directions.
% While a complex kernel with many length scales are prone to overfitting and expensive to train, those with few cannot effectively capture the variations of the high dimensional function in different directions.
% fit the landscapes of the function both in a coordinate subspace and in the full space.  %landscape of the function. 
%
To alleviate this problem, we introduce Coordinate backoff Bayesian Optimization (CobBO) with two-stage kernels.  
%
During each round, the first stage uses a simple coarse kernel that sacrifices the approximation accuracy for computational efficiency. It captures the global landscape by purposely smoothing away local fluctuations. Then, in the second stage of the same round, past observed points in the full space are projected to the selected subspace to form virtual points. 
These virtual points, along with the means and variances of their unknown function values estimated using the simple kernel of the first stage, are fitted to a more sophisticated kernel model in the second stage. Within the selected low dimensional subspace, the computational cost of conducting Bayesian optimization therein becomes affordable. To further enhance the performance, a sequence of consecutive observations in the same subspace are collected, which
can effectively refine the approximation of the function. 
%A more sophisticated kernel is applied to fit these virtual points according to their estimated means and variances from the simple kernel. 
%This is further used to conduct the Bayesian optimization in the selected low dimensional subspace, where the computational cost becomes affordable. 
%In each iteration, a promising subset of coordinates is selected in the first stage, as past observed points in the full space are projected to the selected subspace adopting a simple kernel that sacrifices the approximation accuracy for computational efficiency.
%Then in the second stage of the same iteration a more sophisticated kernel is applied for estimating the landscape in the selected low dimensional subspace where the computational cost becomes affordable. 
%
%Effectively, this second stage refines the approximation of the function estimated by the first stage through a sequence of observations in a subspace. 
%
% Effectively, it refines the approximation of the function through a sequence of observations in a subspace. 
This refinement lasts until a stopping rule is met determining when to back off from a certain subspace and switch to another.
This decoupling significantly reduces the computational burden in high dimensions,
which fully leverages the observations in the whole space rather than only relying on observations in each coordinate subspace.
Extensive evaluations show that CobBO finds solutions comparable to or better than other state-of-the-art methods for dimensions ranging from tens to hundreds, while reducing both the trial complexity and computational costs.
\end{abstract}

==> algorithm/algo_AAAI.tex <==
%\textbf{Algorithm outline:}
% by the virtual points and their smoothed values
%$\hat{\mathcal{H}}_t$ that is generated from the true observations $\mathcal{H}_t$, to approximate $F$. 

\begin{algorithm}[th]
	\caption{Detailed description of CobBO(f, $\tau$, T)}
	\label{alg:top}
\begin{algorithmic}[1] 
\STATE $\mathcal{H}_{\tau} \leftarrow$ sample $\tau$ initial points and evaluate their values\\
\STATE $V_\tau, M_\tau \leftarrow$ the maximal point in $\mathcal{H}_{\tau}$\\
\STATE $q_{\tau} \leftarrow 0$, number of consecutive failed queries\\
\STATE $\pi_{\tau} \leftarrow$ uniform preference for coordinates\\
\FOR{$t \leftarrow \tau\; \mathrm{to}\; T$}
    \IF {
    % \rm{
    switch $\Omega_{t-1}$ by the backoff stopping rule %(Section~\ref{ss:backoff})
    % }
    }
    \STATE $\Omega_t \leftarrow$ Take a new subspace over a coordinate block $C_t$, satisfying $V_t\in \Omega_t$
    \ELSE
       \STATE $\Omega_t \leftarrow \Omega_{t-1}$ //conduct consistent query in the same subspace
    \ENDIF
   \IF{ $\Omega_{t}$ is not $\Omega_{t-1}$}
      \STATE \textbf{Stage 1}: use a simple kernel $K_1$ for the estimation function $R(\cdot, \cdot)$	
   \STATE $\hat{\mathcal{X}}_{t} \leftarrow$ $P_{\Omega_t}(\mathcal{X}_{t})$ 
    //form virtual points %$\mathcal{X}_{t}$
	                   %onto $\Omega_t$ to obtain a set of virtual points (Eq.~\ref{eq:projection})\Big{]}
    \STATE $\hat{\mathcal{H}}_{t} \leftarrow$ $R\left( \hat{\mathcal{X}}_t, \mathcal{H}_t\right)$ //compute the means and variances of the virtual points by $K_1$ 
	                   % \Big{[}Smooth function values on $\hat{\mathcal{X}}_{t}$ by interpolation using $\mathcal{H}_t$\Big{]} 
	\ELSE
	\STATE $\hat{\mathcal{X}}_{t} \leftarrow \hat{\mathcal{X}}_{t-1}$,
	       $\hat{\mathcal{H}}_{t} \leftarrow \hat{\mathcal{H}}_{t-1}$
	       //stage 1 is not needed if remaining in the same subspace
	\ENDIF
\STATE \textbf{Stage 2}: use a sophisticated kernel $K_2$ for BO within $\Omega_t$
\STATE $p\left[ \hat{f}_{\Omega_t}(x) | \hat{\mathcal{H}}_{t} \right] \leftarrow$ Compute the posterior distribution of the Gaussian process in $\Omega_t$ conditional on $\hat{\mathcal{H}}_{t}$ by $K_2$; note that the points in $\hat{\mathcal{H}}_{t}$ could have non-zero variances
\STATE ${x}_{t+1} \leftarrow \textrm{argmax}_{x\in \Omega_t} Q_{ \hat{f} \sim p(\hat{f}|\hat{\mathcal{H}}_t)}(x  | \hat{\mathcal{H}}_t)$ //keep using $K_2$
        %  \Big{[} Suggest the next query in $\Omega_t$ (Section~\ref{sec:algorithm})\Big{]}
\STATE $y_{t+1} = f(x_{t+1})$
% \STATE $y_{t+1} \leftarrow$ Evaluate the black-box function $y_{t+1} = f(x_{t+1})$
\IF{$y_{t+1} > M_t$}
\STATE  $V_{t+1} \leftarrow x_{t+1}$, $M_{t+1} \leftarrow y_{t+1}$, $q_{t+1} \leftarrow 0$
\ELSE
    \STATE $V_{t+1} \leftarrow V_t$, $M_{t+1} \leftarrow M_t$, $q_{t+1} \leftarrow q_t + 1$
\ENDIF 
% \STATE $\pi_{t+1} \leftarrow $ Update $\pi_{t}$ by a multiplicative weights update method (Eq.~\ref{eq:multiplicative_update})
\STATE Update $\pi_{t}$ according to Eq.~\ref{eq:multiplicative_update}
\STATE $\mathcal{H}_{t+1} \leftarrow \mathcal{H}_{t} \bigcup \{(x_{t+1}, y_{t+1})\}$, $\mathcal{X}_{t+1} \leftarrow \mathcal{X}_{t} \bigcup \{x_{t+1}\}$
\ENDFOR 
\end{algorithmic}
\end{algorithm}


==> algorithm/algorithm_1_cobbo.tex <==
%\textbf{Algorithm outline:}
% by the virtual points and their smoothed values
%$\hat{\mathcal{H}}_t$ that is generated from the true observations $\mathcal{H}_t$, to approximate $F$. 

\RestyleAlgo{boxruled}
\LinesNumbered
\vspace{-1.4mm}
\setlength{\dbltextfloatsep}{0pt}
\IncMargin{1.8em}
% \begin{figure*}
% \begin{multicols}{2}
\begin{algorithm*}[tbh]\vspace{1.0mm}
	\SetAlgoLined
	%\textbf{Parameter}: $T =\#$ total trials , $S=\#$ initial samples \\
	%initialization\;
	$\mathcal{H}_{\tau} \leftarrow$ sample $\tau$ initial points and evaluate their values\\
	$V_\tau, M_\tau \leftarrow$ Find the tuple with the maximal objective value in $\mathcal{H}_{\tau}$\\
	$q_{\tau} \leftarrow 0$ Initialize the number of consecutive failed queries\\
	$\pi_{\tau} \leftarrow$ Initialize a uniform preference distribution on the coordinates\\
	\For{$t \leftarrow \tau\; \mathrm{to}\; T$}{
        \uIf{\rm{switch $\Omega_{t-1}$ by the backoff stopping rule (Section~\ref{ss:backoff})}}{ 
	       %     \uIf{\rm{$q_t > \Theta$}}{
        %             % $V_t, M_t \leftarrow$ Sample at random a tuple from the values of $\mathcal{H}_{\tau}$. Pick the furthest away from $V_{t-1}$ (Section~\ref{sec:algorithm})
        %             $V_t, M_t \leftarrow$ Escape local maxima (Section~\ref{ss:escape})] \\
        %             $q_t \leftarrow 0$
        %         }
        %       $K_t \leftarrow$ Update a virtual clock (Eq.~\ref{eq:virtual_clock})\\
        %       $\tilde{\Omega}_t \leftarrow$ Form trust regions on two different time scales (Section~\ref{ss:2tr}) \\
        %       %($K_t$, $y_t$, $M_{t-1}$, $q_t$ %(Algorithm~\ref{alg:trust_region})\\
              $C_t \leftarrow$ Sample a promising coordinate block according to $\pi_t$ (Section~\ref{ss:block})\\
	           $\Omega_t \leftarrow$ Take the subspace of $\Omega_t$ over the coordinate block $C_t$, such that $V_t\in \Omega_t$
	       %   $\Omega_t \leftarrow$ A subspace of $\tilde{\Omega}_t$ over a chosen coordinate block that includes $V_t$ (Section~\ref{ss:key_features})
        }
            \uElse{
    	        $\Omega_t \leftarrow \Omega_{t-1}$
            }
	            
	        $\hat{\mathcal{X}}_{t} \leftarrow$ $P_{\Omega_t}(\mathcal{X}_{t})$ \Big{[}Project $\mathcal{X}_{t}$ 
	                   onto $\Omega_t$ to obtain a set of virtual points (Eq.~\ref{eq:projection})\Big{]}\\
	        $\hat{\mathcal{H}}_{t} \leftarrow$ $R\left( \hat{\mathcal{X}}_t, \mathcal{H}_t\right)$ 
	                    \Big{[}Smooth function values on $\hat{\mathcal{X}}_{t}$ by interpolation using $\mathcal{H}_t$\Big{]}  \\
	        $p\left[ \hat{f}_{\Omega_t}(x) | \hat{\mathcal{H}}_{t} \right] \leftarrow$ Compute the posterior distribution of the Gaussian process in $\Omega_t$ conditional on $\hat{\mathcal{H}}_{t}$ \\
	        %${x}_{t+1} \leftarrow$ $\textrm{argmax}_x  \hat{f}_{\Omega_t}(x, \hat{\mathcal{H}}_{t})$ \Big{[}compute the next query point  in $\Omega_t$ \Big{]}\\
	        ${x}_{t+1} \leftarrow \textrm{argmax}_{x\in \Omega_t} Q_{ \hat{f} \sim p(\hat{f}|\hat{\mathcal{H}}_t)}(x  | \hat{\mathcal{H}}_t)$ 
	                         \Big{[} Suggest the next query in $\Omega_t$ (Section~\ref{sec:algorithm})\Big{]}\\
	        %$\textrm{pivot}_t \leftarrow  \textrm{find} \; x^{+}$ such that $f(x^{+}) \geq  f(x_i), \forall i \in \{1, \cdots, t\}$\\
	        %$x_t \leftarrow$ construct the next query point in $\mathcal{X}$ using $\hat{x}^{\ast}_t$ and $\textrm{pivot}_t$\\
	        $y_{t+1} \leftarrow$ Evaluate the black-box function $y_{t+1} = f(x_{t+1})$\\
            % $\left(V_{t+1}, M_{t+1}\right) \leftarrow \left(x_{t+1}, y_{t+1}\right) \textbf{ if } y_{t+1} > M_t \textbf{ else } \left(V_t, M_t\right)$ [Update the best observed point]\\
            \uIf{$y_{t+1} > M_t$}{
                $V_{t+1} \leftarrow x_{t+1}$, $M_{t+1} \leftarrow y_{t+1}$, $q_{t+1} \leftarrow 0$
            }
            \uElse{
                $V_{t+1} \leftarrow V_t$, $M_{t+1} \leftarrow M_t$, $q_{t+1} \leftarrow q_t + 1$
            }
	        $\pi_{t+1} \leftarrow $ Update $\pi_{t}$ by a multiplicative weights update method (Eq.~\ref{eq:multiplicative_update})\\
	       % $\pi_{t+1} \leftarrow $ MW($\pi_t$, $C_t$, $y_{t+1}$, $M_t$) \Big{[} update $\pi_{t}$ by a multiplicative weights update method\Big{]}\\
	        $\mathcal{H}_{t+1} \leftarrow \mathcal{H}_{t} \bigcup \{(x_{t+1}, y_{t+1})\}$, $\mathcal{X}_{t+1} \leftarrow \mathcal{X}_{t} \bigcup \{x_{t+1}\}$
	        %\eIf{\rm{do drop-out}}
	        %{ conduct robust point filtering
	        %}
	  }
	\caption{CobBO(f, $\tau$, T)}
	\label{alg:top}
\end{algorithm*}

% \end{multicols}
% \end{figure*}

==> algorithm/algorithm_full.tex <==
%\textbf{Algorithm outline:}
% by the virtual points and their smoothed values
%$\hat{\mathcal{H}}_t$ that is generated from the true observations $\mathcal{H}_t$, to approximate $F$. 

\RestyleAlgo{boxruled}
\LinesNumbered
\vspace{-1.4mm}
\setlength{\dbltextfloatsep}{0pt}
\IncMargin{1.8em}
% \begin{figure*}
% \begin{multicols}{2}
\begin{algorithm*}[tbh]\vspace{1.0mm}\label{alg:top}
	\SetAlgoLined
	%\textbf{Parameter}: $T =\#$ total trials , $S=\#$ initial samples \\
	%initialization\;
	$\mathcal{H}_{\tau} \leftarrow$ sample $\tau$ initial points and evaluate their values\\
	$V_\tau, M_\tau \leftarrow$ Find the tuple with the maximal objective value in $\mathcal{H}_{\tau}$\\
	$q_{\tau} \leftarrow 0$ Initialize the number of consecutive failed queries\\
	$\pi_{\tau} \leftarrow$ Initialize a uniform preference distribution on the coordinates\\
	\For{$t \leftarrow \tau\; \mathrm{to}\; T$}{
        \uIf{\rm{switch $\Omega_{t-1}$ by the backoff stopping rule (Section~\ref{ss:backoff})}}{ 
	            \uIf{\rm{$q_t > \Theta$}}{
                    % $V_t, M_t \leftarrow$ Sample at random a tuple from the values of $\mathcal{H}_{\tau}$. Pick the furthest away from $V_{t-1}$ (Section~\ref{sec:algorithm})
                    $V_t, M_t \leftarrow$ Escape local maxima (Section~\ref{ss:escape})] \\
                    $q_t \leftarrow 0$
                }
              $K_t \leftarrow$ Update a virtual clock (Eq.~\ref{eq:virtual_clock})\\
              $\tilde{\Omega}_t \leftarrow$ Form trust regions on two different time scales (Section~\ref{ss:2tr}) \\
              %($K_t$, $y_t$, $M_{t-1}$, $q_t$ %(Algorithm~\ref{alg:trust_region})\\
              $C_t \leftarrow$ Sample a promising coordinate block according to $\pi_t$ (Section~\ref{ss:block})\\
	           $\Omega_t \leftarrow$ Take the subspace of $\tilde{\Omega}_t$ over the coordinate block $C_t$, such that $V_t\in \Omega_t$
	       %   $\Omega_t \leftarrow$ A subspace of $\tilde{\Omega}_t$ over a chosen coordinate block that includes $V_t$ (Section~\ref{ss:key_features})
        }
            \uElse{
    	        $\Omega_t \leftarrow \Omega_{t-1}$
            }
	            
	        $\hat{\mathcal{X}}_{t} \leftarrow$ $P_{\Omega_t}(\mathcal{X}_{t})$ \Big{[}Project $\mathcal{X}_{t}$ 
	                   onto $\Omega_t$ to obtain a set of virtual points (Eq.~\ref{eq:projection})\Big{]}\\
	        $\hat{\mathcal{H}}_{t} \leftarrow$ $R\left( \hat{\mathcal{X}}_t, \mathcal{H}_t\right)$ 
	                    \Big{[}Smooth function values on $\hat{\mathcal{X}}_{t}$ by interpolation using $\mathcal{H}_t$\Big{]}  \\
	        $p\left[ \hat{f}_{\Omega_t}(x) | \hat{\mathcal{H}}_{t} \right] \leftarrow$ Compute the posterior distribution of the Gaussian process in $\Omega_t$ conditional on $\hat{\mathcal{H}}_{t}$ \\
	        %${x}_{t+1} \leftarrow$ $\textrm{argmax}_x  \hat{f}_{\Omega_t}(x, \hat{\mathcal{H}}_{t})$ \Big{[}compute the next query point  in $\Omega_t$ \Big{]}\\
	        ${x}_{t+1} \leftarrow \textrm{argmax}_{x\in \Omega_t} Q_{ \hat{f} \sim p(\hat{f}|\hat{\mathcal{H}}_t)}(x  | \hat{\mathcal{H}}_t)$ 
	                         \Big{[} Suggest the next query point in $\Omega_t$ (Section~\ref{sec:algorithm})\Big{]}\\
	        %$\textrm{pivot}_t \leftarrow  \textrm{find} \; x^{+}$ such that $f(x^{+}) \geq  f(x_i), \forall i \in \{1, \cdots, t\}$\\
	        %$x_t \leftarrow$ construct the next query point in $\mathcal{X}$ using $\hat{x}^{\ast}_t$ and $\textrm{pivot}_t$\\
	        $y_{t+1} \leftarrow$ Evaluate the black-box function $y_{t+1} = f(x_{t+1})$\\
            % $\left(V_{t+1}, M_{t+1}\right) \leftarrow \left(x_{t+1}, y_{t+1}\right) \textbf{ if } y_{t+1} > M_t \textbf{ else } \left(V_t, M_t\right)$ [Update the best observed point]\\
            \uIf{$y_{t+1} > M_t$}{
                $V_{t+1} \leftarrow x_{t+1}$, $M_{t+1} \leftarrow y_{t+1}$, $q_{t+1} \leftarrow 0$
            }
            \uElse{
                $V_{t+1} \leftarrow V_t$, $M_{t+1} \leftarrow M_t$, $q_{t+1} \leftarrow q_t + 1$
            }
	        $\pi_{t+1} \leftarrow $ Update $\pi_{t}$ by a multiplicative weights update method (Eq.~\ref{eq:multiplicative_update})\\
	       % $\pi_{t+1} \leftarrow $ MW($\pi_t$, $C_t$, $y_{t+1}$, $M_t$) \Big{[} update $\pi_{t}$ by a multiplicative weights update method\Big{]}\\
	        $\mathcal{H}_{t+1} \leftarrow \mathcal{H}_{t} \bigcup \{(x_{t+1}, y_{t+1})\}$, $\mathcal{X}_{t+1} \leftarrow \mathcal{X}_{t} \bigcup \{x_{t+1}\}$
	        %\eIf{\rm{do drop-out}}
	        %{ conduct robust point filtering
	        %}
	  }
	\caption{CobBO(f, $\tau$, T)}
\end{algorithm*}

% \end{multicols}
% \end{figure*}

==> algorithm/clock_algo.tex <==
\begin{algorithm}[tbh]\vspace{0.0mm}
    \label{alg:clock}
% 	\SetAlgoLined
    \textbf{Input}: Virtual clock $K_t$ \\
    Relative improvement threshold $\delta$ \\
    Previous best values $M_{t-1}$ \\
    Current observed value $y_t$ \\
    Current and previous points respectively $x_t$, $x_{t-1}$ \\
    $\Delta \leftarrow \frac{y_t - M_{t-1}}{\left|M_{t-1}\right|}$ \\
    \uIf{$\Delta \leq 0$}{
        $K_{t+1} \leftarrow K_t + 1$
      }
      \uElseIf{$0 < \Delta \leq \delta$}{
    	 $\gamma_t \leftarrow \left(1-\frac{\Delta}{\delta}\right) \cdot \left(1 - \frac{||x_t - x_{t-1}||}{\sqrt{|C_t|}} \right)$ \\
        $K_{t+1} \leftarrow \gamma_t \cdot K_t$
      }
      \Else{
        $K_{t+1} \leftarrow 0$
      }
	\caption{UpdateClock($K_t$, $\delta$, $y_t$, $M_{t-1}$, $x_t$, $x_{t-1}$)}
\end{algorithm}

==> algorithm/cobbo_old.tex <==
%\textbf{Algorithm outline:}
% by the virtual points and their smoothed values
%$\hat{\mathcal{H}}_t$ that is generated from the true observations $\mathcal{H}_t$, to approximate $F$. 
\RestyleAlgo{boxruled}
\LinesNumbered
\vspace{-1.4mm}
\IncMargin{1.8em}
% \begin{figure*}
% \begin{multicols}{2}
\begin{algorithm*}[tbh]\vspace{0.0mm}\label{alg:top}
	\SetAlgoLined
	%\textbf{Parameter}: $T =\#$ total trials , $S=\#$ initial samples \\
	%initialization\;
	$\mathcal{H}_S \leftarrow$ use Latin hypercube sampling to get $S$ initial points and evaluate their values\\
	$\pi_S \leftarrow$ initialize a uniform preference distribution on the coordinates\\
	\For{$t \leftarrow S\; \mathrm{to}\; T$}{
	        \eIf{\rm{persistent query [determined by a backoff stopping rule]}}
	             { $\Omega_t \leftarrow \Omega_{t-1}$ }
	             {{ \eIf{\rm{$\#$ consecutive failed queries $\leq$ threshold}}
	                    {$V_t \leftarrow \textrm{argmax}_{x\in \mathcal{X}_t}f(x)$ ; $M_t \leftarrow f\left(V_t\right)$ \Big{[} find the maximum point in observations $\mathcal{X}_t$ \Big{]}}
	                    { $V_t \leftarrow \textrm{random}\{x\in \mathcal{X}_t\}$ ; $M_t \leftarrow f\left(V_t\right)$ \Big{[}  Sample a point in observations $\mathcal{X}_t$ strategically\Big{]}}
	             }
	             { $\Omega_t \leftarrow$ sample a random coordinate subspace containing $V_t$ according to $\pi_{t}$, or\\
	               \hspace{0.8cm} find the top performing coordinates; form a trust region when needed
	            }
	            }
	        $\hat{\mathcal{X}}_{t} \leftarrow$ $P_{\Omega_t}(\mathcal{X}_{t})$ \Big{[}project $\mathcal{X}_{t}$ 
	                   onto $\Omega_t$ to obtain a set of virtual points (Eq.~\ref{eq:projection})\Big{]}\\
	        $\hat{\mathcal{H}}_{t} \leftarrow$ $R\left( \hat{\mathcal{X}}_t, \mathcal{H}_t\right)$ 
	                    \Big{[}smooth function values on $\hat{\mathcal{X}}_{t}$ by RBF interpolation using $\mathcal{H}_t$  ( Eq.~\ref{eq:rbf})\Big{]}  \\
	        $p\left[ \hat{f}_{\Omega_t}(x) | \hat{\mathcal{H}}_{t} \right] \leftarrow$ compute the posterior distribution of the Gaussian process\\
	                     \hspace{2.62cm}conditional on $\hat{\mathcal{H}}_{t}$ within the subspace $\Omega_t$\\
	        %${x}_{t+1} \leftarrow$ $\textrm{argmax}_x  \hat{f}_{\Omega_t}(x, \hat{\mathcal{H}}_{t})$ \Big{[}compute the next query point  in $\Omega_t$ \Big{]}\\
	        ${x}_{t+1} \leftarrow \textrm{argmax}_{x\in \Omega_t} Q_{ \hat{f} \sim p(\hat{f}|\mathcal{H}_t)}(x  | \mathcal{H}_t)$ 
	                         \Big{[} suggest the next query point  in $\Omega_t$ \Big{]}\\
	        %$\textrm{pivot}_t \leftarrow  \textrm{find} \; x^{+}$ such that $f(x^{+}) \geq  f(x_i), \forall i \in \{1, \cdots, t\}$\\
	        %$x_t \leftarrow$ construct the next query point in $\mathcal{X}$ using $\hat{x}^{\ast}_t$ and $\textrm{pivot}_t$\\
	        $y_{t+1} \leftarrow$ evaluate the black-box function $y_{t+1} = f(x_{t+1})$\\
	        $\pi_{t+1} \leftarrow $ update $\pi_{t}$ by a multiplicative weights update method ( Eq.~\ref{eq:multiplicative_update})\\
	       % $\pi_{t+1} \leftarrow $ MW($\pi_t$, $C_t$, $y_{t+1}$, $M_t$) \Big{[} update $\pi_{t}$ by a multiplicative weights update method\Big{]}\\
	        $\mathcal{H}_{t+1} \leftarrow \mathcal{H}_{t} \bigcup \{(x_{t+1}, y_{t+1})\}$, $\mathcal{X}_{t+1} \leftarrow \mathcal{X}_{t} \bigcup \{x_{t+1}\}$
	        %\eIf{\rm{do drop-out}}
	        %{ conduct robust point filtering
	        %}
	  }
	\caption{CobBO(f, S, T)}
\end{algorithm*}
% \end{multicols}
% \end{figure*}

==> algorithm/mw_algo.tex <==
\begin{algorithm}[tbh]\vspace{0.0mm}
    \label{alg:mw}
% 	\SetAlgoLined
    \textbf{Input}: Learning rates $\alpha$, $\beta$ \\
    Coordinate block $C_t$ \\
    Previous best values $M_{t-1}$ \\
    Current observed value $y_t$ \\
    $\pi_{t+1} \leftarrow \pi_t$ \\
	\For{$j \in C_t$}{
        \eIf{$M_t > M_{t-1}$}
             {$\pi_{t+1, j} \leftarrow \pi_{t+1, j} \cdot \alpha$}
             {$\pi_{t+1, j} \leftarrow \pi_{t+1, j} \cdot \beta$}
	  }
	\caption{MW($\pi_t$, $C_t$, $y_t$, $M_{t-1}$)}
\end{algorithm}

==> algorithm/theoretical_analysis_backup.tex <==
\subsection{Theoretical Analysis} \label{ss:analysis}
One can view our block coordinate selection approach in section~\ref{ss:block} as a combinatorial mixture of experts problem~\cite{cesa2006prediction}, where each coordinate is a single expert and the forecaster aims at choosing the best combination of experts in each step. Under this view, we bound the regret of our selection method with respect to the policy of selecting the best (unknown) block of coordinates at each step.

Assume that there is a fixed and optimal choice $C^*$ for the block of coordinates to pick at every step. This block is characterized by improving the objective function the most number of times among all the possible coordinate blocks when performing Bayesian optimization over the corresponding subspaces. The following particular design of losses:
\begin{align} \label{eq:alpha_beta_loss}
    \ell_{t,i} =
    \begin{cases}
		-
        % \frac{1}{\eta}
		\log(\tilde{\alpha}) & \text{if } i \in C_t \text{ and } y_t > M_{t-1} \\
% 		\frac{1}{\eta}
		\log(\tilde{\beta}) & \text{if } i \in C_t \text{ and } y_t \leq M_{t-1} \\
        0 & \text{if } i \notin C_t
    \end{cases} 
    \quad ; \quad 
    \tilde{\alpha},\tilde{\beta}>1
\end{align}
expresses this cause, as all the coordinates participating in the selected block incur the same loss that effectively rewards the coordinates for improving the objective and penalizes for failing to improve the objective. All other coordinates that are not selected receive a zero loss and remain untouched.

Note that $\tilde{\alpha}$ and $\tilde{\beta}$ express the extent of reward and penalty, e.g. for $\tilde{\alpha}=\tilde{\beta}=e$ we have %balanced 
losses of $\ell_{t,i} \in\{-1, 1, 0\}$. %respectively.
% \begin{align} \label{eq:alpha_beta_loss_ones}
%     \ell_{t,i} =
%     \begin{cases}
% 		-
%         % \frac{1}{\eta}
% 		1 & \text{if } i \in C_t \text{ and } y_t > M_{t-1} \\
% % 		\frac{1}{\eta}
% 		1 & \text{if } i \in C_t \text{ and } y_t \leq M_{t-1} \\
%         0 & \text{if } i \notin C_t
%     \end{cases}
% \end{align}
Yet, $\tilde{\alpha}$ is better chosen to be larger than $\tilde{\beta}$, since the frequency of improving the objective is expected to be smaller.%since improving the objective can be rather hard and thus the queries that improve the best observations $y_t > M_{t-1}$ happen more rarely than the opposite $y_t \leq M_{t-1}$. 

The total loss of the forecaster is to express the same motivation. This is done by averaging the losses of the individual coordinates in the selected block, so that the size of the block does not matter explicitly. Such that for each coordinate block $\mathcal{I}_t
\subset\mathcal{I}=\{1,\cdots,D\}$ selected in time step $t$, the loss incurred by the forecaster is:
\begin{equation}
    L_{t,\mathcal{I}_t} =\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} = \bar{\ell}_{t,\mathcal{I}_t}
\end{equation}
where $\bar{\ell}_{t,\mathcal{I}_t}$ is the common loss incurred by all the coordinates participating in that block.

In each step we have the following multiplicative update rule of the weights associated with each coordinate (setting $\alpha=\tilde{\alpha}^\eta$ and $\beta=\tilde{\beta}^\eta$ yields the update rule in Eq. \ref{eq:multiplicative_update}):
 \begin{equation}
    \label{eq:multiplicative_weight_update}
    w_{t, i}
    = 
    w_{t-1, i} \cdot
    \begin{cases}
			\tilde{\alpha}^\eta & \text{if } i \in C_t \text{ and } y_t > M_{t-1} \\
			1/\tilde{\beta}^\eta & \text{if } i \in C_t \text{ and } y_t \leq M_{t-1} \\
            1 & \text{if } i \notin C_t
	 \end{cases} 
	     = w_{t-1, i} \cdot e^{-\eta\ell_{t,i}}
%     \begin{cases}
% 			e^{-\eta\ell_\alpha} & \text{if } j \in C_t \text{ and } y_t > M_{t-1} \\
% 			e^{-\eta\ell_\beta} & \text{if } j \in C_t \text{ and } y_t \leq M_{t-1} \\
%             e^{-\eta\ell_0} & \text{if } j \notin C_t
% 	 \end{cases} 
 \end{equation}

% This particular choice of losses corresponds to rewarding selected coordinates that eventually improve the objective, penalizing selected coordinates that fail to improve the objective and remaining coordinates that are not selected untouched.

Denote all possible block sizes by $\mathcal{C}$ and the set of all possible coordinate blocks of size $c\in\mathcal{C}$ by $\mathcal{S}_c$ and its size $|\mathcal{S}_c|={D \choose c}$. Denote by $p_c$ the probability of choosing a certain block size $c\in\mathcal{C}$, such that $p_c\geq 0$ and $\sum_{c\in\mathcal{C}}p_c=1$. The expected cumulative loss following our update policy is
% Denote all possible block sizes by $\mathcal{C}$ and the set of all possible coordinate blocks by $\mathcal{S}$ and its size $|\mathcal{S}|=\sum_{c\in\mathcal C} {D \choose c}$. The expected cumulative loss following our update policy is
% $$L_T= \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i}$$
$$L_T= \sum_{t=1}^T\sum_{c\in\mathcal{C}}p_c\sum_{\mathcal{I}_t\in \mathcal{S}_c}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i}$$
where the probability $\hat{\pi}_{t,\mathcal{I}_t}$ of selecting a certain coordinate block $\mathcal{I}_t$ follows sampling according to $\pi_t$ without replacement (explicitly put in Appendix~\ref{sec:regret_analysis}).

Assume the best coordinate block is $C^*$ and the corresponding cumulative loss:
$$L_T^*= \sum_{t=1}^T L_{t,\mathcal{I}_t}=\sum_{t=1}^T\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} = \sum_{t=1}^T\bar{\ell}_{t,\mathcal{I}_t}$$

We hence aim at bounding the regret $Regret_T = L_T-L_T^*$. For this purpose we bound the regret with respect to any arbitrary sequence of selected coordinate blocks.

\textbf{Lemma 1} Assume $\mathcal{C}\supset\{1\}$ and $p_1>0$. For $\eta >0$ and non-negative losses $\ell_{t,i}\geq 0$ the update rule in (\ref{eq:multiplicative_weight_update}) satisfies for any block of coordinates $C^*$:
\begin{equation}\label{eq:lemma_1}
Regret_T
% =L_T-L^*_T 
% =
% \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} - \sum_{t=1}^T \ell^*_t
%  \sum_{t=1}^T\sum_{c\in\mathcal{C}}p_c\sum_{\mathcal{I}_t\in \mathcal{S}_c}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} - \sum_{t=1}^T \ell^*_t
\leq 
\eta\sum_{t=1}^T\sum_{c\in\mathcal{C}}p_c\sum_{\mathcal{I}_t\in \mathcal{S}_c}\hat{\pi}_{t,\mathcal{I}_t}\cdot \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 + \frac{\log(D)}{\eta} -\frac{T\log(p_1)}{\eta}
\end{equation}
% where $p_1$ is the probability of sampling a block of size $1$. 
And thus we bound the regret (the proofs are in Appendix \ref{sec:regret_analysis}):\\
\textbf{Theorem 1} The update in Eq.~\ref{eq:multiplicative_update}, with $\alpha=\tilde{\alpha}^\eta$, $\beta=\tilde{\beta}^\eta$ and
$\eta=\sqrt{\frac{\log(D)}{T(\log(\tilde{\alpha}\tilde{\beta})^2 -\log(p_1))}}\geq 1$ yields:
 \begin{equation}\label{eq:regret}
     Regret_t 
     \leq 
      \mathcal{O}\left(\sqrt{(\log(\tilde{\alpha}\tilde{\beta})^2 -\log(p_1))} \cdot \sqrt{T\log(D)})\right)
 \end{equation}
 The regret upper bound in Eq.~\ref{eq:regret} is tight, as the lower bound for an easier setup can be shown to be of $\Omega(\sqrt{T\log(D)})$ \cite{haussler1995tight}. 
 The implication on $\eta$ is valid only for settings of a very high dimensionality and low query budget. In particular, CobBO is designed %to do well 
 for this kind of problems. 
% Moreover, interestingly, although the effective number of combinations of coordinates is $|\mathcal{S}|\leq  |\mathcal{C}|\cdot(D!)$, the regret upper bound in \ref{eq:regret} shows to grow with $\mathcal{O}(\sqrt{\log(D)})$ rather than $\mathcal{O}(\sqrt{\log(|\mathcal{C}|)+\log(D!)})\sim\mathcal{O}(\sqrt{D\log(D)})$ for large $D>>|\mathcal{C}|$ due to the Stirling's approximation~\cite{pearson1924historical}. This is due to adapting the preference probability $\pi_{t,i}$ for each coordinate rather than the one for each possible combination of coordinates $\hat{\pi}_{t,\mathcal{I}_t}$, as the later is derived from the former.

==> algorithm/trust_region_algo.tex <==
% \algnewcommand{\IfThenElse}[3]{% \IfThenElse{<if>}{<then>}{<else>}
%   \State \algorithmicif\ #1\ \algorithmicthen\ #2\ \algorithmicelse\ #3}
  
\begin{algorithm}[tbh]\vspace{0.0mm}
    \label{alg:trust_region}
% 	\SetAlgoLined
    % \textbf{Input}: Current virtual Clock $K_t$\\
    \textbf{Parameters}: \\
    \hspace{0.5cm} Slow/fast thresholds $\kappa_{S/F}$ respectively\\
    \hspace{0.5cm} Slow/fast cycles $\tau_{S/F}$ respectively\\
    % Current observed value $y_t$ \\
    % Previous best value $M_{t-1}$ \\
    % Consecutive fails to improve $q_t$ \\
    \textbf{Init}: $\Omega_{S_0}, \Omega_{F_0} \leftarrow \Omega$ \\
    \uIf{$y_t > M_{t-1}$} {
        $\Omega_{S_t}, \Omega_{F_t} \leftarrow$ Double $\Omega_{S_{t-1}}$ around $V_t$% at each coordinate
    }
    \uElseIf{$mod\left(K_t, \kappa_S\right) = 0$}{
        $\Omega_{S_t} \leftarrow$ Halve $\Omega_{S_{t-1}}$ around $V_t$% at each coordinate
    }
    \uElse{
        $\Omega_{S_t} \leftarrow \Omega_{S_{t-1}}$
    }
    
    \uIf{$mod\left(q_t, \kappa_F\right) = 0$}{
        $\Omega_{F_t} \leftarrow$ Halve $\Omega_{F_{t-1}}$ around $V_t$% at each coordinate
    } 
    % \textbf{Alternation}:\\
    \uIf{$mod\left(q_t, \tau_S+\tau_F\right) < \tau_S$}{
         $\tilde{\Omega}_{t} \leftarrow \Omega_{S_t}$
     }
    \uElse{
         $\tilde{\Omega}_t \leftarrow \Omega_{F_t}$
    }
    % $\tilde{\Omega}_{t} \leftarrow \Omega_{S_t} \textbf{ If } mod\left(q_t, \tau_S+\tau_F\right) < \tau_S\textbf{ Else } \Omega_{F_t}\$
    % \IfThenElse {$mod\left(q_t, \tau_S+\tau_F\right) < \tau_S$}% If ...
    %   {$\Omega_{S_t}$}% ...then...
    %   {$\Omega_{F_t}$}% ...else...
      
    \textbf{Output}: Trust Region $\tilde{\Omega}_{t}$
	\caption{FormTrustRegions($K_t$,$y_t$,$M_{t-1}$,$q_t$)}
% 	\caption{FormTrustRegionsPolicy($K_t$, $\kappa_S$, $\kappa_F$, $\tau_S$, $\tau_F$, $y_t$, $M_{t-1}$, $q_t$)}
\end{algorithm}
\setlength{\textfloatsep}{0pt}

% \begin{algorithm}[tbh]\vspace{0.0mm}
%     \label{alg:trust_region}
% % 	\SetAlgoLined
%     \textbf{Input}: Current virtual Clock $K_t$\\
%     Slow/fast thresholds $\kappa_{S/F}$ respectively\\
%     % Fast threshold $\kappa_f$,\\
%     Slow/fast cycles $\tau_{S/F}$ respectively\\
%     Current observed value $y_t$ \\
%     Previous best values $M_{t-1}$ \\
%     Consecutive fails to improve $q_t$ \\
%     $\Omega_{S_0}, \Omega_{F_0} \leftarrow \Omega$ \\
   
%     \For{$B \in \{S, F\}$}{
%         \uIf{$y_t > M_{t-1}$}{
%             % $\Omega_{B_t} \leftarrow$ \Big{[}Enlarge $\Omega_{B_{t-1}}$ by doubling the space around $V_t$ at each coordinate\Big{]}
%             $\Omega_{B_t} \leftarrow$ Double $\Omega_{B_{t-1}}$ around $V_t$ at each coordinate
%         }
%         \uElseIf{$mod\left(K_t, \kappa_B\right) = 0$}{
%             % $\Omega_{B_t} \leftarrow$ \Big{[}Shrink $\Omega_{B_{t-1}}$ by halving the space around $V_t$ at each coordinate\Big{]}
%             $\Omega_{B_t} \leftarrow$ Halve $\Omega_{B_{t-1}}$ around $V_t$ at each coordinate
%         }
%         \uElse{
%             $\Omega_{B_t} \leftarrow \Omega_{B_{t-1}}$
%         }
%     }
    
%     \uIf{$mod\left(q_t, \tau_S+\tau_F\right) < \tau_S$}{
%          $\tilde{\Omega}_{t} \leftarrow \Omega_{S_t}$
%      }
%     \uElse{
%          $\tilde{\Omega}_t \leftarrow \Omega_{F_t}$
%     }
%     \textbf{Output}: Trust Region $\tilde{\Omega}_{t}$
% 	\caption{TrustRegionsPolicy($K_t$, $\kappa_S$, $\kappa_F$, $\tau_S$, $\tau_F$, $y_t$, $M_{t-1}$, $q_t$)}
% \end{algorithm}

% \begin{algorithm}[tbh]\vspace{0.0mm}
%     \label{alg:trust_region_2}
%     \textbf{Input}: Current virtual Clock $K_t$\\
%     Slow/fast thresholds $\kappa_{S/F}$ respectively\\
%     % Fast threshold $\kappa_f$,\\
%     Alternating cycle $\tau$\\
%     Current observed value $y_t$ \\
%     Previous best values $M_{t-1}$ \\
%     Consecutive fails to improve $q_t$ \\
% % 	\SetAlgoLined
%     % \quad ; \quad
%     % r \leftarrow mod\left(K_t, \kappa_S\right)$ \\
%     \For{$B \in \{S, F\}$}{
%         $n \leftarrow \floor{\frac{K_t}{\kappa_B}}$ \\
%     	\For{$d = 1,\dots, D$}{
%             $l^{(d)} \leftarrow \max\left(0, V_t^{(d)} - \frac{1}{2^{n}}\right)$ \\
%             $u^{(d)} \leftarrow \min\left(1, V_t^{(d)} + \frac{1}{2^{n}}\right)$ \\
%             $\Omega_B^{(d)} \leftarrow [l^{(d)}, u^{(d)}]$
%         }      
%     }
    
%     \uIf{$mod\left(q_t, \tau\right) = 0$}{
%         \uIf{$\tilde{\Omega} = \Omega_S$}{
%              $\tilde{\Omega} \leftarrow \Omega_F$
%         }
%         \uElse{
%              $\tilde{\Omega} \leftarrow \Omega_S$
%         }
%     }
%     \textbf{Output}: Trust Region $\tilde{\Omega}$
% 	\caption{TrustRegionsPolicy($K_t$, $\kappa_S$, $\kappa_F$, $\tau$, $y_t$, $M_{t-1}$, $q_t$)}
% \end{algorithm}

==> broader_impact.tex <==
\section*{Broader Impact}
As stated in~\cite{letham2020re}, Bayesian optimization is a powerful optimization technique used in a wide range of industries and applications, such as robotics~\cite{lizotte2007automatic,calandra2016bayesian,rai2018bayesian}, internet tech companies~\cite{golovin2017google,letham2019constrained}, designing novel molecules for pharmaceutics~\cite{gomez2018automatic}, material design for increasing efficiency of solar cells~\cite{zhang2020bayesian}, and aerospace engineering~\cite{lam2018advances}. All of these settings have high-dimensional optimization problems, and advances
in BO will reflect on improved capabilities on these fields as well. We have fully open-sourced our
code for CobBO using the MIT license to be available for researchers and practitioners in these fields, and many others.
The ability to optimize a larger number of parameters than has previously been possible will bring further improvements to and further accelerate work in these areas.

==> experiments/experiments_2.tex <==


% \begin{figure*}[!h]%\vspace{-2mm}
%   \centering
%   \includegraphics[width=0.85
%   \linewidth,height=!]{low_v.png}\vspace{-3mm}
% %   \includegraphics{synthetic.png}\vspace{-3mm}
%   \caption{Performance over low dimensional problems: Ackley (left), Levy (middle) and Rastrigin (right)}
%   \label{fig:synthetic}
% \end{figure*}

%\vspace{-1.5mm}
\section{Numerical Experiments}\label{sec:num_exp}
\input{ablation/ablation}




%\vspace{-2.0mm}
\subsection{Comparisons with other methods}\label{s:exp}
%\vspace{-1.5mm}
%After tuning the hyper-parameters of CobBO over a number of commonly used benchmarks, we fix 
The default configuration for CobBO
is configured with the default settings and hyperparameters for all the experiments, which are specified in the supplementary materials. 
% together with more experiments. 
%Following the same default configuration, 
CobBO performs on par or outperforms a collection of state-of-the-art methods across the following experiments. %This further demonstrates the robustness of CobBO.
%\niv{What is the "default setting" ? The begining of the experiments section is a good place to specify those.}
 %We use extensive experiments to demonstrate the performance of CobBO in both trial complexity and time complexity, 
%all conducted with the default setting. 
%Although CobBO has a number of parameters, it is proven to be robust to those.
%\niv{Where is the robustness to parameters is 'proven' ? Reference to some experiment ?}
%For example, CobBO uses a default setting to allocate the number of initial points ($8\%$ of the total budget, capped at $500$), 
%unless it is explicitly specified. 
Most of the experiments are conducted using the same settings as in TurBO~\cite{turbo2019}, where it is compared with a comprehensive list of baselines, including BFGS, BOCK~\cite{bock2018}, BOHAMIANN~\cite{bohamiann}, CMA-ES~\cite{cmaes}, BOBYQA, EBO~\cite{wang18aistats}, GP-TS, HeSBO~\cite{chaudhuri2019}, Nelder-Mead and random search. 
To avoid repetitions, we only show TuRBO and CMA-ES that achieve the best performance among this list, and additionally compare CobBO with BADS~\cite{luigi2017}, % HDBBO~\cite{zi2017}, SIR~\cite{miao2019},
Differetial Evolution (Diff-Evo)~\cite{storn1997differential},
Tree Parzen Estimator (TPE)~\cite{TPE2011} and Adaptive TPE (ATPE)~\cite{ATPE}. 
Comparisons with REMBO~\cite{ziyuw2016} are presented in Appendix E.2.

%The python code of the experiments and implementation of CobBO will be made publicly available.
%We repeat each experiment independently for 30 times to get the 95\% confidence intervals. 
%, and d-KG~\cite{wujian2017}.
%Though LineBO~\cite{linebo} and DROPOUT~\cite{dropoutbo} are also based on subspace selection,
%they do not show comparable performance.  
%Confidence intervals are computed with the results of 30 independent experiments.


%To overcome this limitation, the recent approach BOHB [33] combines Bayesian optimization and HyperBand 
%to achieve the best of both worlds: strong anytime performance (quick improvements in the beginning by using 
%low fidelities in HyperBand) and strong final performance (good performance in the long run by replacing HyperBand’s 
%random search by Bayesian optimization).


%and SigOpt~\cite{sigopt}. 
%SigOpt has an online black-box optimization service without disclosing its underlying algorithm details. 
% In addition to the benchmarks tested in~\cite{turbo2019}, we also provide new benchmarks,
%including deep neural network and industrial melting.  These benchmarks cover a wide spectrum of applications.
%BOBYAQ, BFGS, Nelder-Mead.
%\subsection{The effect of initial sampling}
%Traditionally initial sampling is conducted through random sampling. 





\begin{figure*}[htb]%\vspace{-2mm}
\begin{center}
  %\includegraphics[width=0.9\linewidth,height=!]{figures/low_mid_high_200d_fixed.pdf}%
  \includegraphics[width=0.98\linewidth,height=!]{figures/low_medium_high_100}%
  \vspace{-5mm}
%   \includegraphics{lunar-robot.png}
\end{center}
  \caption{Performance over low (left) medium (middle) and high (right) dimensional problems}
  \label{fig:low_medium_high}\vspace{0.0mm}
%   \vspace{5mm}
\end{figure*}


%\vspace{-1.5mm}
\subsubsection{Low-dimensional tests:}\label{ss:lowDtest}
%\vspace{-1.5mm}
 To evaluate CobBO on low dimensional problems, we use the lunar landing~\cite{turbo2019}, robot pushing~\cite{wang18aistats} and synthetic functions by following the setup in~\cite{turbo2019}. Confidence intervals ($95\%$) over $30$ independent experiments for each problem are shown in Fig.~\ref{fig:low_medium_high}.
 
 \vspace{0.25cm}
\noindent \emph{Lunar landing (maximization):}
This controller learning problem ($12$ dimensions) is provided by the OpenAI gym and evaluated in~\cite{turbo2019}.
%The controller of a lunar lander decides whether or not to fire the booster engine and the firing direction during landing,   
%based on the current status of the lander in each frame. 
%The average performance of the controller is evaluated by simulations over %a fixed constant set of 
%50 randomly generated terrains and initial states. 
Each algorithm has $50$ initial points and a budget of $1,500$ trials. 
TuRBO is configured with $5$ trust regions and a batch size of $50$ as in~\cite{turbo2019}.   
Fig.~\ref{fig:low_medium_high} (upper left) shows that, among the $30$ independent tests, CobBO quickly exceeds $300$ along some good sample paths.  % outperforming other algorithms. 

% \begin{figure*}[htb]%\vspace{-2mm}
% \begin{center}
%   \includegraphics[width=0.75\linewidth,height=!]{lunar-robot.png}\vspace{-3mm}
% %   \includegraphics{lunar-robot.png}
% \end{center}
%   \caption{Performance over the more complicated lunar landing (left) and robot pushing (right) problems}
%   \label{fig:lunar-robot}
% \end{figure*}
% \begin{figure}[htb]\vspace{-2mm}
% \begin{center}
%   \includegraphics[width=0.75\columnwidth,height=!]{low_hard_v.png}\vspace{-3mm}
% %   \includegraphics{lunar-robot.png}
% \end{center}
%   \caption{Performance over the lunar landing (upper) and robot pushing (lower) problems}\vspace{2mm}
%   \label{fig:lunar-robot}
% \end{figure}


\vspace{0.25cm}
\noindent \emph{Robot pushing (maximization):}
This control problem (14 dimensions) is introduced in~\cite{wang18aistats} and extensively tested in~\cite{turbo2019}. We follow the setting in~\cite{turbo2019}, where TuRBO is configured with a batch size of $50$ and $15$ trust regions, each of which has $30$ initial points. 
%We exclude REMBO that consumes more than $24$ hours per run.  
Each experiment has a budget of $10,000$ evaluations.
On average CobBO exceeds $10$ within $5500$ trials,
%while TuRBO requires about $7000$, 
as shown in Fig. ~\ref{fig:low_medium_high} (lower left).
%Some CobBO runs even get close to 11.0 within 6,000 evaluations. 
%TPE and ATPE converge to around $9$, outperforming BADS and CEM-ES by large margins. 
%The latter two exhibit large variations and get stuck in local optima.

% CobBO finds the best results for the robot pushing problem, 
% slightly outperforming TuRBO, as shown in Fig. ~\ref{fig:control-additive}. 
% Both TPE and ATPE  are less competitive but still outperform BADS and CMA-ES with large margins. 
% The latter two algorithms show large variations and get stuck in suboptima at very early stages.

\vspace{0.25cm}
\noindent \emph{Low-dimensional synthetic black-box functions (minimization):} Three additional synthetic $10$ dimensional functions~\cite{TestProblems2013} are experimented with in Fig.~\ref{fig:synthetic}, including Ackley over $[-5, 10]^{10}$, Levy over $[-5, 10]^{10}$ and Rastrigin over $[-3, 4]^{10}$.
%, and Hartmann(6D) with domain $[0, 1]^{6}$
%Each experiment has a budget of $500$ evaluations. 
TuRBO is configured the same as in~\cite{turbo2019}, with a batch size of $10$ and $5$ concurrent trust regions where each has $10$ initial points. 
The other algorithms use $20$ initial points. The results are shown in Fig.~\ref{fig:synthetic}. CobBO shows competitive or better performance.
It finds the best optima on Ackley and Levy among all the algorithms and outperforms the others for the difficult Rastrigin function. 
Notably, BADS is more suitable for low dimensions, as commented in~\cite{luigi2017}. Its performance is close to CobBO except for Rastrigin. 
%TuRBO performs better than TPE and worse than BADS. ATPE outperforms TPE. 
%CMA-ES eventually catches up with TPE, ATPE and REMBO on Ackley.
%REMBO appears unstable with large variations and is trapped in local optima. 
\begin{figure}[!ht]%\vspace{-2mm}
  \centering
  \includegraphics[width=0.95
  \linewidth,height=!]{figures/low_v.png}\vspace{-3mm}
%   \includegraphics{synthetic.png}\vspace{-3mm}
  \caption{Low dimensional problems: Ackley (left), Levy (middle) and Rastrigin (right)}
  \label{fig:synthetic}\vspace{0mm}
\end{figure}

In Fig.~\ref{fig:micha} we show that CobBO also optimizes well the Michalewicz function on $10$ dimensions, although it has symmetric bumps, where certain subspaces pass through a point in a symmetrical manner and others break it. 
\begin{figure}[!htb]
  \centering
    \includegraphics[width=0.45\textwidth]{ICML/michal.png}
     \caption{Performance over the low dimensional Michalewicz function with symmetrical and asymmetrical subspaces} 
    \label{fig:micha}
\end{figure}
Other real applications include parameter tuning for recommendation systems, database online performance tuning, and simulation based parameter optimization. However, due to deviating from the main study of this paper, we refrain from presenting these results that require elaborated description on the application backgrounds. 


\vspace{0.25cm}
\noindent \emph{Medium-sized synthetic black-box functions (minimization):}
We test three synthetic functions ($30$ dimensions), including Ackley on $[-5, 10]^{30}$, Levy $[-5, 10]^{30}$, and Rastrigin on $[-3, 4]^{30}$. In addition, 
we add experiments for an additive function of $36$ dimensions, defined as  $f_{36}(x)=\rm{Ackley}(x_1) + \rm{Levy}(x_2) + \rm{Rastrigin}(x_3) + \rm{Hartmann}(x_4)$, where the first three terms express the same functions over the same domains specified in Section~3.1 of this paper, with the Hartmann function over $[0, 1]^{6}$. 
TuRBO is configured identically the same as in Section~3.1, with a batch size of 10 and 5 trust regions with 10 initial points each. The other algorithms use 20 initial points.
The results are shown in Fig.~\ref{fig:30D-tests} and~\ref{fig:additive-36D}, where CobBO shows competitive or better performance compared to all of the methods tested across all of these problems.
 \begin{figure}[!htb]\vspace{-0mm}
   \centering
   \includegraphics[width=0.8\columnwidth,height=!]{supplementary/additive-36D.png}%\vspace{1mm}
   \caption{Performance over an additive function of 36 dimensions}%\vspace{5mm}
   \label{fig:additive-36D}
 \end{figure}


 
 



%\vspace{-1.5mm}
\subsubsection{High dimensional tests:}
Since each experiment takes a long time, confidence intervals ($95\%$) over repeated $10$ independent experiments for each problem are presented.

\noindent \emph{Additive latent structure (minimization):}
As mentioned in 
%the related work
Section~\ref{sec:related_work}, additive latent structures have been exploited %for tackling challenges 
in high dimensions.
%which however incur a high computational cost~\cite{chaudhuri2019}.   %For $x=(x_1, x_2, x_3, x_4)$,  
We construct an additive function of $56$ dimensions, defined as $f_{56}(x) = \rm{Ackley}(x_1) + \rm{Levy}(x_2) + \rm{Rastrigin}(x_3) + \rm{Hartmann}(x_4) +\rm{Rosenbrock}(x_5)+\rm{Schwefel}(x_6)$, where the first three terms express the exact functions and domains described in Section~\ref{ss:lowDtest}, the Hartmann function on $[0, 1]^{6}$ and the Rosenbrock and Schwefel functions on $[-5,10]^{10}$ and $[-500,500]^{10}$, respectively. 

We compare CobBO with TPE, BADS, CMA-ES and TuRBO, each with $100$ initial points. 
% and a budget of 5,000 evaluations. 
Specifically, TuRBO is configured with $1$ trust region and a batch size $100$. 
ATPE is excluded as it takes more than 24 hours per run to finish. 
%The other algorithms have a budget of 10,000 evaluations for $f_{56}$. The experiment setup is the same as for $f_{36}$, 
%except that the batch size of TuRBO is set to 100. 
The results are shown in Fig.~\ref{fig:low_medium_high} (upper middle), where CobBO quickly finds the best solution among those.
Comparisons with REMBO~\cite{ziyuw2016} are presented in Appendix E.2.
%the algorithms tested.

%As shown in Fig.~\ref{fig:control-additive}, CobBO finds the best solutions for both $f_{36}$  and $f_{56}$. 
%BADS performs closely to CobBO. ATPE outperforms TPE, TuRBO and CMA-ES on $f_{36}$. 
%TuRBO surpasses TPE and CMA-ES on $f_{36}$ eventually, while TPE and CMA-ES converge faster than TuRBO on $f_{56}$.

% \begin{figure*}[htb]\vspace{-2mm}
% \begin{center}
%   \includegraphics[width=1.0\linewidth,height=!]{highDims.png}
% %   \includegraphics{highDims.png}
% \end{center}
%   \caption{Performance over medium-size dimensional problems: 36D (left) and 56D (middle) additive functions and the 60D rover trajectory planning (right)}%\vspace{-1.5mm}
%   \label{fig:highDims}
% \end{figure*}
% \begin{figure}[htb]\vspace{-2mm}
% \begin{center}
%   \includegraphics[width=0.75\columnwidth,height=!]{medium_v.png}\vspace{-3mm}
% %   \includegraphics{highDims.png}
% \end{center}
%   \caption{Performance over medium-size dimensional problems: 56D additive functions (upper) and the 60D rover trajectory planning (lower)}\vspace{-1.5mm}
%   \label{fig:highDims}
% \end{figure}

\noindent \emph{Rover trajectory planning (maximization):} 
This problem (60 dimensions) is introduced in~\cite{wang18aistats}. 
The objective is to find a collision-avoiding trajectory of a sequence consisting of 30 positions in a 2-D plane. 
%$[0,1]^{2}$. 
We compare CobBO with TuRBO, TPE and CMA-ES, each with a budget of $20,000$ evaluations and $200$ initial points. 
TuRBO is configured with $15$ trust regions and a batch size of $100$, as in~\cite{turbo2019}. 
ATPE, BADS and REMBO are excluded for this problem and the following ones, as they all take more than 24 hours per run. 
%The results are shown in 
Fig.~\ref{fig:low_medium_high} (lower middle) shows that CobBO has a good performance. 
%quickly reaches the best solution.
%among the tested algorithms faster than TuRBO, while TPE and CMA-ES reach inferior solutions.

\noindent \emph{The 100-dimensional Levy and Rastrigin functions (minimization):} %\label{sec:100d}
We minimize the Levy and Rastrigin functions on $[-5, 10]^{100}$ with $500$ initial points. 
TuRBO is configured with $15$ trust regions and a batch size of $100$.
As commented in~\cite{turbo2019}, these two problems are challenging and have no redundant dimensions. 
 Fig.~\ref{fig:100d} (left) shows that CobBO can greatly reduce the trial complexity. 
 For Levy, it finds solutions close to the final one within $1,000$ trials, and eventually reach the best solution among all the algorithms tested.
 For Rastrigin, within $2,000$ trials CobBO and TuRBO surpass the final solutions of all the other methods, eventually with a large margin.
 
 %\clearpage
  \begin{figure}[!htb]
   \centering
   \includegraphics[width=0.8\columnwidth,height=!]{figures/synth_100d.pdf}
   \caption{Performance over high dimensional synthetic problems: Levy (left) and Rastrigin (right)}
   \label{fig:100d} %\vspace{5mm}
 \end{figure}
 
  For high dimensional problems, REMBO is too slow for almost all of the tested problems and gives bad results. For Ackley 200D with $4000$ iterations, REMBO and CobBO reach the mean best values of $15.1$ and $3.8$, respectively, running for $31.2$ and $3.4$ hours, respectively. %With the effective dimension of REMBO set to $20$ (similarly to CobBO, whose average is about 15). 
  This shows that CobBO outperforms REMBO by a large margin, and requires about $10\%$ of the computation time for this experiment.


%\vspace{0.5mm}
\noindent \emph{The 200-dimensional Levy and Ackley functions (minimization):}
We minimize the Levy and Ackley functions over $[-5, 10]^{200}$ with $500$ initial points. 
TuRBO-1 is configured with $1$ trust region and a batch size of $100$.
These two problems are challenging and have no redundant dimensions. 
 For Levy, in Fig.~\ref{fig:low_medium_high} (upper right), CobBO reaches $100$ within $2,000$ trials, while CMA-ES and TuRBO 
 obtain $200$ after $8,000$ trials. TPE cannot find a comparable solution within $10,000$ trials in this case. 
 For Ackley, in Fig.~\ref{fig:low_medium_high} (lower right), TuRBO, CMA-ES and CobBO converge to the mean best values of $4.53$, $3.33$ and $2.91$ respectively after $20,000$ trials. To be consistent with Levy, we present the first $10,000$ steps that also highlight the effectiveness of CobBO at relatively low query budgets for high dimensional functions. %CobBO reaches the best solution among all of the algorithms tested. 
%  The appealing trial complexity of CobBO suggests that it can be applied in a hybrid method, e.g., used in the first stage of the query process combined with gradient estimation methods or CMA-ES.

Regarding running times, for a fair comparison, we change the configure so that both TurBO and CobBO have the same batch size of $1$. For Ackley, CobBO runs for $12.8$ CPU hours and TuRBO-1 runs for more than $80$ CPU hours or $9.6$ \emph{GPU} hours. Other methods either cannot make any progress or find far worse solutions.


\subsubsection{Comparison to LineBO}\label{ss:linebo}
 Although sharing some common basic ideas, LineBO~\cite{linebo} reduces the acquisition maximization cost by restricting on a line but does not reduce the expensive computational costs of the GP regression in the full space. Fig.~\ref{fig:linebo} shows that LineBO is significantly outperformed by CobBO through a typical example in $D=10$ (Ackely). 
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth, height=!]{ICML/linebo_ackley}
   \caption{A typical example of CobBO outperforming different variants of LineBO}
   \label{fig:linebo}
\end{figure}
In another typical experiment of $D=30$ and a query budget of 5000, CobBO reached 0.12 and LineBO reached 7.6. 

\subsubsection{Comparison to ALEBO}\label{ss:alebo}
ALEBO~\cite{letham2020} is designed for high-dimensional (large $D$) problems with low intrinsic dimensions (small $d$). For comparison, we first test CobBO using exactly the same setting as in~\cite{letham2020} for Hartmann6 with $D=1000$ dimensions and only $d=6$ intrinsic dimensions, as shown in Fig.~\ref{fig:hart6}. 
%We also test on problems without the assumption on
%such sparsities or a priori knowledge about the exact 
Then, for the general problems without the assumption on low intrinsic dimensions, we test ALEBO on Ackley(10D) in three sets of experiments in Fig.~\ref{fig:alebo}, where $D=d=10$. Since ALEBO algorithm requires to provide a low intrinsic dimension $d<D$, we test $d=2,4,8$ dimensions (i.e., ALEBO-2, ALEBO-4, and ALEBO-8), respectively. 
Fig.~\ref{fig:hart6} and~\ref{fig:alebo} show
the final results by repeating each experiment $30$ times.


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.55\textwidth, height=!]{supplementary/hart1000.pdf}
  \caption{Performance on Hartmann6 ($D=1000$, $d=6$)}
  \label{fig:hart6}
\end{figure}
For the first case, ALEBO indeed outperforms CobBO, since CobBO is not designed for a function with a low effective dimension, i.e.,  $f(x) = g(\Phi x)$ for a function $g(\cdot)$ and a matrix $\Phi$ of $d\times D, d<<D$, which essentially assumes that $f(x)$ does not change along certain directions. 


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.32\textwidth, height=!]{supplementary/ackley10-alebo-2.pdf}
    \includegraphics[width=0.32\textwidth, height=!]{supplementary/ackley10-alebo-4.pdf}
    \includegraphics[width=0.32\textwidth, height=!]{supplementary/ackley10-alebo-8.pdf}
  \caption{Compare ALEBO and CobBO on Ackley(10D)}
  \label{fig:alebo}
\end{figure}
%However, it takes ALEBO $12$ hours on average and only $10$ minutes for CobBO to finish the experiment.
For the second case, ALEBO does not show good performance and is outperformed by CobBO, TurBO and CMAES. 
% Regarding the computation times, it takes $6$ to $12$ hours for ALEBO and only $3$ minutes for CobBO to finish $500$ queries for each experiment on our testbed for the second case. 





 %Confidence intervals ($95\%$) are computed by repeating 10 independent experiments for each problem, as shown in Fig.~\ref{fig:200d}.
%  \begin{figure*}[htb]\vspace{-2mm}
%   \centering
%   \includegraphics[width=0.98\linewidth,height=!]{levy200d.png}\vspace{-3mm}
% %   \includegraphics{levy200d.png}\vspace{-3mm}
% \caption{Performance over high dimensional problems: the 200D Levy (left) and Ackley (middle) functions and the 102D half-cheetah control problem (right)}\vspace{-1.5mm}
%   \label{fig:200d}
%  \end{figure*}
%  \begin{figure}[htb]\vspace{-2mm}
%   \centering
%   \includegraphics[width=0.75\columnwidth,height=!]{high_v.png}\vspace{-3mm}
% %   \includegraphics{levy200d.png}\vspace{-3mm}
% \caption{Performance over high dimensional problems: the 200D Levy (upper) and Ackley (upper) functions}\vspace{-5mm}
%   \label{fig:200d}
%  \end{figure}


%\textbf{Half-cheetah control problem (maximization):}
%This is a model-free reinforcement learning problem ($102$ dimensions) provided by OpenAI gym~\cite{cheetah}.
% to  maximize the accumulated rewards.
%It has been shown that Augmented Random Search~\cite{mania2018,ars}, a random search method based on gradient estimation, in conjunction with a linear control policy, can achieve state-of-the-art sample efficiency and a competitive performance. 
% We apply the linear control policy as in~\cite{mania2018,ars}, governed by 102 unknown parameters to be searched over $[-0.1,0.1]^{102}$. The results in Fig.~\ref{fig:200d} demonstrate that Bayesian optimization can also efficiently find comparable solutions.
% \niv{Comparable to what ? what is the baseline score ?}
 





 




==> experiments/experiments_long.tex <==
\vspace{-1.5mm}
\section{Numerical experiments}\label{s:exp}
\vspace{-1.5mm}
After tuning the hyper-parameters of CobBO over a number of commonly used benchmarks, we fix a default configuration for CobBO to be used across all of the experiments. The values are specified in the supplementary materials together with more experiments. Following the same default configuration, CobBO performs on par or outperforms a collection of state-of-the-art methods across the following experiments. This further demonstrates the robustness of CobBO.
%\niv{What is the "default setting" ? The begining of the experiments section is a good place to specify those.}
 %We use extensive experiments to demonstrate the performance of CobBO in both trial complexity and time complexity, 
%all conducted with the default setting. 
%Although CobBO has a number of parameters, it is proven to be robust to those.
%\niv{Where is the robustness to parameters is 'proven' ? Reference to some experiment ?}
%For example, CobBO uses a default setting to allocate the number of initial points ($8\%$ of the total budget, capped at $500$), 
%unless it is explicitly specified. 
Most of the experiments are conducted using the same settings as in TurBO~\cite{turbo2019}, where it is compared with a comprehensive list of baselines, including BFGS, BOCK~\cite{bock2018}, BOHAMIANN, CMA-ES~\cite{cmaes}, BOBYQA, EBO~\cite{wang18aistats}, GP-TS, HeSBO~\cite{chaudhuri2019}, Nelder-Mead and random search. 
To avoid repetitions, we only show TuRBO and CMA-ES that achieve the best performance among this list, and additionally compare CobBO with BADS~\cite{luigi2017},  REMBO~\cite{ziyuw2016}, % HDBBO~\cite{zi2017}, SIR~\cite{miao2019},
Tree Parzen Estimator (TPE)~\cite{TPE2011} and Adaptive TPE (ATPE)~\cite{ATPE}. 
The python code of the experiments will be made publicly available, together with the implementation of CobBO.
%We repeat each experiment independently for 30 times to get the 95\% confidence intervals. 
%, and d-KG~\cite{wujian2017}.
%Though LineBO~\cite{linebo} and DROPOUT~\cite{dropoutbo} are also based on subspace selection,
%they do not show comparable performance.  
%Confidence intervals are computed with the results of 30 independent experiments.


%To overcome this limitation, the recent approach BOHB [33] combines Bayesian optimization and HyperBand 
%to achieve the best of both worlds: strong anytime performance (quick improvements in the beginning by using 
%low fidelities in HyperBand) and strong final performance (good performance in the long run by replacing HyperBand’s 
%random search by Bayesian optimization).


%and SigOpt~\cite{sigopt}. 
%SigOpt has an online black-box optimization service without disclosing its underlying algorithm details. 
% In addition to the benchmarks tested in~\cite{turbo2019}, we also provide new benchmarks,
%including deep neural network and industrial melting.  These benchmarks cover a wide spectrum of applications.
%BOBYAQ, BFGS, Nelder-Mead.
%\subsection{The effect of initial sampling}
%Traditionally initial sampling is conducted through random sampling. 

\vspace{-1.5mm}
\subsection{Low dimensional tests}\label{ss:lowDtest}
\vspace{-1.5mm}
 To evaluate the performance of CobBO on low dimensional problems, we use classic synthetic black-box functions~\cite{TestProblems2013}, as well as two more challenging problems of lunar landing~\cite{lunar,turbo2019}  and robot pushing~\cite{wang2018robotpush}, by following the setup in~\cite{turbo2019} for most experiments. Confidence intervals ($95\%$) over repeated 30 independent experiments for each problem are shown.
 
\textbf{Classic synthetic black-box functions (minimization):}
Three popular synthetic functions ($10$ and $30$ dimensions) are chosen, including Ackley over $[-5, 10]^{10}$ and $[-5, 10]^{30}$, Levy over both $[-5, 10]^{10}$ and $[-5, 10]^{30}$, and Rastrigin over both $[-3, 4]^{10}$ and $[-3, 4]^{30}$.
%, and Hartmann(6D) with domain $[0, 1]^{6}$
%Each experiment has a budget of $500$ evaluations. 
TuRBO is configured identically the same as in~\cite{turbo2019}, with a batch size of $10$ and $5$ concurrent trust regions where each has $10$ initial points. 
%\niv{What does it mean "$5$ trust regions" ?}
The other algorithms use $20$ initial points. The results are shown in Fig.~\ref{fig:synthetic}. CobBO shows competitive or better performance for all of these problems.
It finds the global optima on Ackley and Levy, and clearly outperforms the other algorithms for the difficult Rastrigin function. 
Notably, BADS is more suitable for low dimensions, as commented in~\cite{luigi2017}, which performs close to CobBO except on Rastrigin. 
TuRBO performs better than TPE and worse than BADS. ATPE outperforms TPE. % and is close to CobBO on Levy.
CMA-ES eventually catches up with TPE, ATPE and REMBO on Ackley.
REMBO appears unstable with large variations and is trapped at local optima. 
For the $30$-dimensional problems and the following experiments, REMBO is excluded as it takes more than 24 hours per experiment. 
\begin{figure*}[htb]\vspace{-2mm}
  \centering
  \includegraphics[width=0.98\linewidth,height=!]{synthetic.png}\vspace{-3mm}
%   \includegraphics{synthetic.png}\vspace{-3mm}
  \caption{Performance over 10D (top) and 30D (bottom) synthetic black-box functions: Ackley (left), Levy (middle) and Rastrigin (right)}\vspace{-1.5mm}
  \label{fig:synthetic}
\end{figure*}

%\textbf{The 30-dimensional classic functions:}
%We compare CobBO with TuRBO, BADS, TPE, ATPE and CMA-ES on the 30 dimensional versions of the Ackley, Levy and Rastrigin functions 
%introduced in Section \ref{ss:lowDtest}. %(except the Hartmann function that is defined to be fixed 6 dimensional)
%
%As shown in Fig. ~\ref{fig:synthetic}, CobBO finds the global optima of Ackley the Levy, and the best results for Rastrigin. 
%BADS is competitive with CobBO on Ackley and Levy, while it performs next to CobBO on Rastrigin.  
%CMA-ES outperforms TuRBO, TPE and ATPE on Ackley, and is comparable to TPE on the other two problems. 

 
\textbf{Lunar landing (maximization):}
This controller learning problem ($12$ dimensions) is provided by the OpenAI gym~\cite{lunar}  
and evaluated in~\cite{turbo2019}.
%The controller of a lunar lander decides whether or not to fire the booster engine and the firing direction during landing,   
%based on the current status of the lander in each frame. 
%The average performance of the controller is evaluated by simulations over %a fixed constant set of 
%50 randomly generated terrains and initial states. 
Each algorithm has 50 initial points and a budget of $1,500$ trials. 
TuRBO is configured with 5 trust regions and a batch size of 50 as in~\cite{turbo2019}.   
Fig.~\ref{fig:lunar-robot} shows that, among the $30$ independent tests, CobBO quickly exceeds $300$ along some good sample paths.  % outperforming other algorithms. 

\begin{figure*}[htb]%\vspace{-2mm}
\begin{center}
  \includegraphics[width=0.75\linewidth,height=!]{lunar-robot.png}\vspace{-3mm}
%   \includegraphics{lunar-robot.png}
\end{center}
  \caption{Performance over the more complicated lunar landing (left) and robot pushing (right) problems}
  \label{fig:lunar-robot}
\end{figure*}

\textbf{Robot pushing (maximization):}
This control problem (14 dimensions) is introduced in~\cite{wang2018robotpush} and extensively tested in~\cite{turbo2019}.  We follow the setting in~\cite{turbo2019}, where TuRBO is configured with a batch size of 50 and 15 trust regions where each has 30 initial points.  
%We exclude REMBO that consumes more than $24$ hours per run.  
Each experiment has a budget of $10,000$ evaluations.
On average CobBO exceeds 10.0 within 5,500 trials, while TuRBO requires about 7,000, 
as shown in Fig. ~\ref{fig:lunar-robot}.
%Some CobBO runs even get close to 11.0 within 6,000 evaluations. 
TPE and ATPE converge to around 9.0, outperforming BADS and CEM-ES with large margins. 
The latter two exhibit large variations and get stuck at local optima.



% CobBO finds the best results for the robot pushing problem, 
% slightly outperforming TuRBO, as shown in Fig. ~\ref{fig:control-additive}. 
% Both TPE and ATPE  are less competitive but still outperform BADS and CMA-ES with large margins. 
% The latter two algorithms show large variations and get stuck in suboptima at very early stages.

\vspace{-1.5mm}
\subsection{High dimensional tests}
\vspace{-1.5mm}
Since the duration of each experiment in this section is long, confidence intervals ($95\%$) over repeated 10 independent experiments for each problem are shown.

\textbf{Additive latent structure (minimization):}
As mentioned in the related work (section~\ref{sec:related_work}), additive latent structures have been explored for tackling challenges in high dimensions.
%which however incur a high computational cost~\cite{chaudhuri2019}.   %For $x=(x_1, x_2, x_3, x_4)$,  
We construct two additive functions. The first one has 36 dimensions, defined as  
 $f_{36}(x)=\rm{Ackley}(x_1) + \rm{Levy}(x_2) + \rm{Rastrigin}(x_3) + \rm{Hartmann}(x_4)$, where the first three terms express the exact functions and domains described in Section~\ref{ss:lowDtest},  with the Hartmann function defiend over $[0, 1]^{6}$. 
 The second has 56 dimensions, defined as 
 $f_{56}(x) = \rm{Ackley}(x_1) + \rm{Levy}(x_2) + \rm{Rastrigin}(x_3) + \rm{Hartmann}(x_4) +\rm{Rosenbrock}(x_5)+\rm{Schwefel}(x_6)$, 
 where the first four terms are the same as those of $f_{36}$, with the Rosenbrock and Schwefel functions defined over $[-5,10]^{10}$ and $[-500,500]^{10}$, respectively. 

We compare CobBO with TPE, ATPE, BADS, CMA-ES and TuRBO, each with $100$ initial points. 
% and a budget of 5,000 evaluations. 
Specifically, TuRBO is configured with 15 trust regions and a batch size 50 for $f_{36}$ and $100$ for $f_{56}$. 
ATPE is excluded for $f_{56}$ as it takes more than 24 hours per run to finish. 
%The other algorithms have a budget of 10,000 evaluations for $f_{56}$. The experiment setup is the same as for $f_{36}$, 
%except that the batch size of TuRBO is set to 100. 
The results are shown in Fig.~\ref{fig:highDims}, where CobBO quickly finds the best solutions for both $f_{36}$  and $f_{56}$.


%As shown in Fig.~\ref{fig:control-additive}, CobBO finds the best solutions for both $f_{36}$  and $f_{56}$. 
%BADS performs closely to CobBO. ATPE outperforms TPE, TuRBO and CMA-ES on $f_{36}$. 
%TuRBO surpasses TPE and CMA-ES on $f_{36}$ eventually, while TPE and CMA-ES converge faster than TuRBO on $f_{56}$.

% \begin{figure*}[htb]\vspace{-2mm}
% \begin{center}
%   \includegraphics[width=1.0\linewidth,height=!]{highDims.png}
% %   \includegraphics{highDims.png}
% \end{center}
%   \caption{Performance over medium-size dimensional problems: 36D (left) and 56D (middle) additive functions and the 60D rover trajectory planning (right)}%\vspace{-1.5mm}
%   \label{fig:highDims}
% \end{figure*}
% \begin{figure}[htb]\vspace{-2mm}
% \begin{center}
%   \includegraphics[width=0.75\columnwidth,height=!]{medium_v.png}\vspace{-3mm}
% %   \includegraphics{highDims.png}
% \end{center}
%   \caption{Performance over medium-size dimensional problems: 56D additive functions (upper) and the 60D rover trajectory planning (lower)}\vspace{-1.5mm}
%   \label{fig:highDims}
% \end{figure}

\textbf{Rover trajectory planning (maximization):} 
This problem (60 dimensions) is introduced in~\cite{wang2018robotpush}. 
The objective is to find a collision-avoiding trajectory of a sequence consisting of 30 positions in a 2-D plane. 
%$[0,1]^{2}$. 
We compare CobBO with TuRBO, TPE and CMA-ES with a budget of $20,000$ evaluations and
$200$ initial points. 
TuRBO is configured with $15$ trust regions and a batch size of $100$, as in~\cite{turbo2019}. 
ATPE, BADS and REMBO are excluded for this problem and the following ones, as they all last for more than 24 hours per run. The result is shown in Fig.~\ref{fig:highDims}. CobBO reaches the best solution faster than TuRBO, while TPE and CMA-ES reach inferior solutions.

 \textbf{The \textcolor{red}{200-dimensional Levy and Ackley} functions (minimization):}
We minimize the Levy and Ackley functions over $[-5, 10]^{200}$ with $500$ initial points. 
As commented in~\cite{turbo2019},
 these two problems are challenging and have no redundant dimensions. 
 Fig.~\ref{fig:200d} shows that CobBO can dramatically
 reduce the trial complexity. 
 For Levy, it quickly finds solutions close to the optimal within $1,000$ trials. 
 All of the other tested algorithms take more than $10,000$ trials and still cannot obtain a comparable solution. 
 For Ackley, CobBO reaches 4.0 within $1,800$ trials, while CMA-ES requires $7,000$ trials. 
 TuRBO 
 \textcolor{red}{(with a batch size of 100 \cite{turbo2019})}  and TPE cannot find a comparable solution within $10,000$ trials. 
 %The appealing trial complexity of CobBO suggests that it can be applied in a hybrid method, 
 %e.g., used in the first stage of the query process when combined with gradient estimation methods or CMA-ES.
  Furthermore, note that CobBO's sample variance for the Levy function across $10$ independent experiments is extremely low, as can be seen in Fig.~\ref{fig:200d}. % for the tested algorithms. 
 %Confidence intervals ($95\%$) are computed by repeating 10 independent experiments for each problem, as shown in Fig.~\ref{fig:200d}.
%  \begin{figure*}[htb]\vspace{-2mm}
%   \centering
%   \includegraphics[width=0.98\linewidth,height=!]{levy200d.png}\vspace{-3mm}
% %   \includegraphics{levy200d.png}\vspace{-3mm}
% \caption{Performance over high dimensional problems: the 200D Levy (left) and Ackley (middle) functions and the 102D half-cheetah control problem (right)}\vspace{-1.5mm}
%   \label{fig:200d}
%  \end{figure*}
%  \begin{figure}[htb]\vspace{-2mm}
%   \centering
%   \includegraphics[width=0.75\columnwidth,height=!]{high_v.png}\vspace{-3mm}
% %   \includegraphics{levy200d.png}\vspace{-3mm}
% \caption{Performance over high dimensional problems: the 200D Levy (upper) and Ackley (upper) functions}\vspace{-5mm}
%   \label{fig:200d}
%  \end{figure}


%\textbf{Half-cheetah control problem (maximization):}
%This is a model-free reinforcement learning problem ($102$ dimensions) provided by OpenAI gym~\cite{cheetah}.
% to  maximize the accumulated rewards.
%It has been shown that Augmented Random Search~\cite{mania2018,ars}, a random search method based on gradient estimation, in conjunction with a linear control policy, can achieve state-of-the-art sample efficiency and a competitive performance. 
% We apply the linear control policy as in~\cite{mania2018,ars}, governed by 102 unknown parameters to be searched over $[-0.1,0.1]^{102}$. The results in Fig.~\ref{fig:200d} demonstrate that Bayesian optimization can also efficiently find comparable solutions.
% \niv{Comparable to what ? what is the baseline score ?}
 





 




==> regret/regret_analysis_backup.tex <==
\section{Regret Analysis} \label{sec:regret_analysis}
In this section we provide proofs for the theorems in Sec.~\ref{ss:analysis}.

Following Eq.~\ref{eq:multiplicative_update}, at every step a probability distribution is induced over the coordinates $\pi_t$:
\begin{align}
    \pi_{t,i} = \frac{w_{t,i}}{W_t} \quad \text{where} \quad W_t = \sum_{i=1}^D w_{t,i}
\end{align}
The probability $\hat{\pi}_{t,\mathcal{I}_t}$ of selecting a certain coordinate block $\mathcal{I}_t\subset \mathcal{I}=\{1,\cdots,D\}$ follows sampling according to $\pi_t$ without replacement, such that,
\begin{align}
    \hat{\pi}_{t,\mathcal{I}_t} 
    &= \sum_{p\in perm(\mathcal{I}_t)} \prod_{k\in p}{\frac{\pi_{t,k}}{1-\sum_{j\in p_{1:k}}\pi_{t,j}}} 
    \\&= \label{eq:common_numerator}
    \left(\prod_{i\in \mathcal{I}_t}\pi_{t,k}\right) \cdot \left(\sum_{p\in perm(\mathcal{I}_t)} \prod_{k\in p}\left(1-\sum_{j\in p_{1:k}}\pi_{t,j}\right)^{-1}\right)
    =
    \mathcal{P}(\mathcal{I}_t) \cdot \mathcal{R}(\mathcal{I}_t)
\end{align}
where $perm(\mathcal{I}_t)$ are all the permutations of the set $\mathcal{I}_t$ and $p_{1:k}$ are the first $k$ coordinates in the permutation $p$. \ref{eq:common_numerator} is due to the common numerator of all permutations where the left term $\mathcal{P}(\mathcal{I}_t)$ corresponds to the probability of sampling a subset of coordinates with replacement, and the right term $\mathcal{R}(\mathcal{I}_t)$ is associated with sampling without replacement.

% Denote the set of all possible coordinate blocks of all sizes $c\in\mathcal{C}$ by $\mathcal{S}$ and its size $|\mathcal{S}|=\prod_{c\in\mathcal C} {D \choose c}$.

% The expected cumulative loss following our update policy is
% $$L_T= \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i}$$

% Assume the best coordinate block is $C^*$ and the corresponding cumulative loss:
% $$L_T^*= \sum_{t=1}^T L_{t,\mathcal{I}_t}=\sum_{t=1}^T\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} = \sum_{t=1}^T\bar{\ell}_{t,\mathcal{I}_t}$$

% We hence aim at bounding the regret $Regret_T = L_T-L_T^*$ 
% For this purpose we bound the regret with respect to any arbitrary sequence of selected coordinate blocks.

% \textbf{Lemma 1} For $\eta >0$ and assume all losses $\ell_t,i \geq 0$ for all $t\in\{1,\cdots,T\}$ and $i\in \mathcal{I}$ the update rule in \ref{eq:multiplicative_weight_update} satisfies for any block of coordinates $C^*$:
% \begin{equation}\label{eq:lemma_1}
% % Regret_T=L_T-L^*_T =
% \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} - \sum_{t=1}^T \ell^*_t
% \leq \eta \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 + \frac{\log(D)}{\eta}
% \end{equation}

In addition, let us first modify the losses in Eq.~\ref{eq:alpha_beta_loss} to be non-negative by adding the same constant $\log(\alpha)$ to all possible values
\begin{align} \label{eq:alpha_beta_loss_shifted}
    \tilde{\ell}_{t,i} =
    \begin{cases}
		0 & \text{if } i \in C_t \text{ and } y_t > M_{t-1} \\
		\log(\tilde{\alpha}\tilde{\beta}) & \text{if } i \in C_t \text{ and } y_t \leq M_{t-1} \\
        \log(\tilde{\alpha}) & \text{if } i \notin C_t
    \end{cases}
\end{align}
This modification does not change the resulted distribution $\pi_t$ induced over the coordinates as it is invariant to shifts of the losses:
\begin{align}
\notag
\pi_{t,i} = \frac{w_{t,i}}{W_t} &= \frac{e^{-\eta\sum_{\tau=1}^t\tilde{\ell}_{\tau,i}}}{\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t\tilde{\ell}_{\tau,j}}} =
\frac{e^{-\eta\sum_{\tau=1}^t(\ell_{\tau,i}+\log(\tilde{\alpha}))}}{\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t(\ell_{\tau,j}+\log(\tilde{\alpha}))}}
=
\frac{e^{-\eta t\log(\tilde{\alpha})}e^{-\eta\sum_{\tau=1}^t\ell_{\tau,i}}}{e^{-\eta t\log(\tilde{\alpha})}\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t\ell_{\tau,j}}}
\\&=
\frac{e^{-\eta\sum_{\tau=1}^t\ell_{\tau,i}}}{\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t\ell_{\tau,j}}}
\end{align}
Thus for simplicity we refer to $\tilde{\ell}$ as $\ell$ in the followings.

% \textbf{Proof} 
\subsection{Proof of Lemma 1}
Starting with a uniform distribution over the coordinates $w_{0,i}\equiv \frac{1}{D}$ such that $W_0 = 1$ and we have:
\begin{align}
    W_{t+1} &= \sum_{i\in \mathcal{I}} w_{t+1,i} 
    \\ & \leq \label{eq:sum_of_products}
    \sum_{\mathcal{I}_t\in \mathcal{S}}\prod_{i\in\mathcal{I}_t}w_{t+1,i}
    \\&=
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}W_t^{-1}\prod_{i\in\mathcal{I}_t}w_{t,i}e^{-\eta\ell_{t,i}} 
    \\&\leq \label{eq:sum_leq_1}
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}W_t^{-|\mathcal{I}_t|}\prod_{i\in\mathcal{I}_t}w_{t,i}e^{-\eta\ell_{t,i}} \cdot|perm(\mathcal{I}_t)|
    \\&=
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\prod_{i\in\mathcal{I}_t}\frac{w_{t,i}}{W_t}e^{-\eta\ell_{t,i}}\cdot \sum_{p\in perm(\mathcal{I}_t)}1 
    \\&=
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\prod_{i\in\mathcal{I}_t}\pi_{t,i}e^{-\eta\ell_{t,i}}\cdot \sum_{p\in perm(\mathcal{I}_t)}\prod_{k\in p}1 
    \\&\leq 
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}e^{-\eta\sum_{i\in\mathcal{I}_t}\ell_{t,i}}\prod_{i\in\mathcal{I}_t}\pi_{t,i}\cdot\sum_{p\in perm(\mathcal{I}_t)}\prod_{k\in p}\left(1-\sum_{j\in p_{1:k}}\pi_{t,j}\right)^{-1}
    \\&= \label{eq:back_to_pi_hat}
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}e^{-\eta\sum_{i\in\mathcal{I}_t}\ell_{t,i}}
    \\&\leq 
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}e^{-\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}}
    \\&\leq \label{eq:exp_ineq}
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\left(1-\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}+\eta^2\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2\right)
    \\&\leq \label{eq:pi_hat_sums_to_1}
    W_t\left(|\mathcal{C}|+\sum_{\mathcal{I}_t\in \mathcal{S}}\eta^2\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)
    \\&\leq 
    W_t\left(1+ (|\mathcal{C}|-1)+\sum_{\mathcal{I}_t\in \mathcal{S}}\eta^2\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)
    \\&\leq \label{eq:exp_ineq_2}
    W_t e^{\sum_{\mathcal{I}_t\in \mathcal{S}} \eta^2|\hat{\pi}_{t,\mathcal{I}_t}\hat{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\hat{\pi}_{t,\mathcal{I}_t}\hat{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i}+(|\mathcal{C}|-1)} 
\end{align}
Where
\begin{itemize}
    \item (\ref{eq:sum_of_products}) is since $\mathcal{C}$ always contains a block size of $1$, i.e. $1\in\mathcal{C}$ and thus: 
    \begin{align*}
        \sum_{\mathcal{I}_t\in \mathcal{S}}\prod_{i\in\mathcal{I}_t}w_{t+1,i}
        &=
        \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\prod_{i\in\mathcal{I}_t}w_{t+1,i}
        \\ &=
        \sum_{\mathcal{I}_t\in\mathcal{S}_1}\prod_{i\in\mathcal{I}_t}w_{t+1,i}+\sum_{c\in\mathcal{C}\setminus \{1\}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\prod_{i\in\mathcal{I}_t}w_{t+1,i}
        \\&=
        \sum_{i\in \mathcal{I}} w_{t+1,i} + \sum_{c\in\mathcal{C}\setminus \{1\}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\prod_{i\in\mathcal{I}_t}w_{t+1,i} 
        \\ & \geq 
        \sum_{i\in \mathcal{I}} w_{t+1,i}
    \end{align*}
    \item (\ref{eq:sum_leq_1}) holds since $W_0=1$ and $W_t$ is monotonically non-increasing following the update rule (\ref{eq:multiplicative_weight_update}) with non-negative losses, thus $w_t\leq 1$ for all $t$.
    \item (\ref{eq:back_to_pi_hat}) follows from (\ref{eq:common_numerator}).
    \item (\ref{eq:exp_ineq}) holds since $e^x\leq 1-x+x^2$ for all $x\geq 0$.
    \item (\ref{eq:pi_hat_sums_to_1}) holds since $\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}=\sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c }\hat{\pi}_{t,\mathcal{I}_t}=\sum_{c\in\mathcal{C}}1=|\mathcal{C}|$.
    \item (\ref{eq:exp_ineq_2}) holds since $1+x\leq e^x$.
\end{itemize}

Given that the sum of weights of a certain coordinate block $C^*$ is less than the total sum of weights, together with Eq.~\ref{eq:exp_ineq_2}, $w_{0,i}\equiv\frac{1}{D}$ and $W_0=1$ we have:
\begin{align}
   \frac{1}{D}\sum_{i\in C^*}e^{-\eta\sum_{t=1}^T\ell_{t,i}}
   = \sum_{i\in C^*} w_{t,i} \leq W_T 
   \leq 
    e^{\sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}} \eta^2\hat{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\hat{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i} + (|\mathcal{C}|-1)} 
\end{align}
Taking the $\log$ of both sides, we have:
\begin{align} \label{eq:recursive_ineq}
  \log&\left(\sum_{i\in C^*}e^{-\eta\sum_{t=1}^T\ell_{t,i}}\right) 
  -\log(D) 
  \notag \\ &\leq \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}} \eta^2\hat{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\hat{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i} 
  + T(|\mathcal{C}|-1)
\end{align}
Following the same certain block, all the participating coordinates suffer the same loss 
 $\ell^*_t$ at every time step as follows from Eq.~\ref{eq:alpha_beta_loss}, hence:
 \begin{align} \notag
     \log\left(\sum_{i\in C^*}e^{-\eta\sum_{t=1}^T\ell_{t,i}}\right)
     &=
     \log\left(\sum_{i\in C^*}e^{-\eta\sum_{t=1}^T\ell^*_t}\right)
     \\ & = \notag
     \log\left(|C^*|e^{-\eta\sum_{t=1}^T\ell^*_t}\right)
     \\&=  \notag
     \log(|C^*|) -\eta\sum_{t=1}^T\ell^*_t
     \\ &\geq \label{eq:common_loss_ineq}
     -\eta\sum_{t=1}^T\ell^*_t
 \end{align}
 Thus Eq.~\ref{eq:recursive_ineq} and \ref{eq:common_loss_ineq} yield:
 \begin{align}
     -\eta|\mathcal{C}|\sum_{t=1}^T\ell^*_t 
     -|\mathcal{C}|\log(D) 
     \leq \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}} \eta^2\hat{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\hat{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i}
     + T\log(|\mathcal{C}|)
 \end{align}
 And since $\sum_{\mathcal{I}_t\in\mathcal{S}}$ is equivalent to $\sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}$, we have:
 \begin{align}
    \sum_{t=1}^T\sum_{c\in\mathcal{C}}&\frac{1}{|\mathcal{C}|}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} - \sum_{t=1}^T \ell^*_t
    \notag \\ & \leq 
    \eta \sum_{t=1}^T\sum_{c\in\mathcal{C}}\frac{1}{|\mathcal{C}|}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\hat{\pi}_{t,\mathcal{I}_t}\cdot \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 + \frac{\log(D)+T(1-1/|\mathcal{C}|)}{\eta} 
 \end{align}
 
 
%  \textbf{Theorem 1}  Apply the update rule in \ref{eq:multiplicative_weight_update}, with a modified $\eta=\log(\alpha\beta)^{-1}\sqrt{\frac{\log(D)}{T}}$, then:
%  \begin{equation*}
%      Regret_t = \mathcal{O}(\log(\alpha\beta)\sqrt{T\log(D)})
%  \end{equation*}
 
%  \textbf{Proof} 
\subsection{Proof of Theorem 1}
 Since $\ell_{t,i} \leq \log(\tilde{\alpha}\tilde{\beta})$ then: 
 \begin{align}
     \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2
     \leq
     \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\log(\tilde{\alpha}\tilde{\beta})\right)^2
     \leq
     \log(\tilde{\alpha}\tilde{\beta})^2
 \end{align}
 
 Thus since $\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}=|\mathcal{C}|$ we have,
 \begin{align}
     \sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2
     \leq
     \sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\log(\tilde{\alpha}\tilde{\beta})^2
     =
     |\mathcal{C}|\log(\tilde{\alpha}\tilde{\beta})^2
 \end{align}
 And Eq.~\ref{eq:lemma_1} yields,
 \begin{equation}
     Regret_t \leq \eta T \log(\tilde{\alpha}\tilde{\beta})^2 
     + \frac{\log(D)+T(1-1/|\mathcal{C}|)}{\eta} 
    %  = 2 \log(\tilde{\alpha}\tilde{\beta})\sqrt{T\log(D)}
 \end{equation}

==> regret/regret_analysis_linear_T.tex <==
\section{Regret Analysis} \label{sec:regret_analysis}
In this section we provide proofs for the theorems in Sec.~\ref{ss:analysis}.

Following Eq.~\ref{eq:multiplicative_update}, at every step a probability distribution is induced over the coordinates $\pi_t$:
\begin{align}
    \pi_{t,i} = \frac{w_{t,i}}{W_t} \quad \text{where} \quad W_t = \sum_{i=1}^D w_{t,i}
\end{align}
The probability $\hat{\pi}_{t,\mathcal{I}_t}$ of selecting a certain coordinate block $\mathcal{I}_t\subset \mathcal{I}=\{1,\cdots,D\}$ follows sampling according to $\pi_t$ without replacement, such that,
\begin{align}
    \hat{\pi}_{t,\mathcal{I}_t} 
    &= \sum_{p\in perm(\mathcal{I}_t)} \prod_{k\in p}{\frac{\pi_{t,k}}{1-\sum_{j\in p_{1:k}}\pi_{t,j}}} 
    \\&= \label{eq:common_numerator}
    \left(\prod_{i\in \mathcal{I}_t}\pi_{t,k}\right) \cdot \left(\sum_{p\in perm(\mathcal{I}_t)} \prod_{k\in p}\left(1-\sum_{j\in p_{1:k}}\pi_{t,j}\right)^{-1}\right)
    =
    \mathcal{P}(\mathcal{I}_t) \cdot \mathcal{R}(\mathcal{I}_t)
\end{align}
where $perm(\mathcal{I}_t)$ are all the permutations of the set $\mathcal{I}_t$ and $p_{1:k}$ are the first $k$ coordinates in the permutation $p$. \ref{eq:common_numerator} is due to the common numerator of all permutations where the left term $\mathcal{P}(\mathcal{I}_t)$ corresponds to the probability of sampling a subset of coordinates with replacement, and the right term $\mathcal{R}(\mathcal{I}_t)$ is associated with sampling without replacement.

% Denote the set of all possible coordinate blocks of all sizes $c\in\mathcal{C}$ by $\mathcal{S}$ and its size $|\mathcal{S}|=\prod_{c\in\mathcal C} {D \choose c}$.

% The expected cumulative loss following our update policy is
% $$L_T= \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i}$$

% Assume the best coordinate block is $C^*$ and the corresponding cumulative loss:
% $$L_T^*= \sum_{t=1}^T L_{t,\mathcal{I}_t}=\sum_{t=1}^T\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} = \sum_{t=1}^T\bar{\ell}_{t,\mathcal{I}_t}$$

% We hence aim at bounding the regret $Regret_T = L_T-L_T^*$ 
% For this purpose we bound the regret with respect to any arbitrary sequence of selected coordinate blocks.

% \textbf{Lemma 1} For $\eta >0$ and assume all losses $\ell_t,i \geq 0$ for all $t\in\{1,\cdots,T\}$ and $i\in \mathcal{I}$ the update rule in \ref{eq:multiplicative_weight_update} satisfies for any block of coordinates $C^*$:
% \begin{equation}\label{eq:lemma_1}
% % Regret_T=L_T-L^*_T =
% \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} - \sum_{t=1}^T \ell^*_t
% \leq \eta \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 + \frac{\log(D)}{\eta}
% \end{equation}

In addition, let us first modify the losses in Eq.~\ref{eq:alpha_beta_loss} to be non-negative by adding the same constant $\log(\alpha)$ to all possible values
\begin{align} \label{eq:alpha_beta_loss_shifted}
    \tilde{\ell}_{t,i} =
    \begin{cases}
		0 & \text{if } i \in C_t \text{ and } y_t > M_{t-1} \\
		\log(\tilde{\alpha}\tilde{\beta}) & \text{if } i \in C_t \text{ and } y_t \leq M_{t-1} \\
        \log(\tilde{\alpha}) & \text{if } i \notin C_t
    \end{cases}
\end{align}
This modification does not change the resulted distribution $\pi_t$ induced over the coordinates as it is invariant to shifts of the losses:
\begin{align}
\notag
\pi_{t,i} = \frac{w_{t,i}}{W_t} &= \frac{e^{-\eta\sum_{\tau=1}^t\tilde{\ell}_{\tau,i}}}{\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t\tilde{\ell}_{\tau,j}}} =
\frac{e^{-\eta\sum_{\tau=1}^t(\ell_{\tau,i}+\log(\tilde{\alpha}))}}{\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t(\ell_{\tau,j}+\log(\tilde{\alpha}))}}
=
\frac{e^{-\eta t\log(\tilde{\alpha})}e^{-\eta\sum_{\tau=1}^t\ell_{\tau,i}}}{e^{-\eta t\log(\tilde{\alpha})}\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t\ell_{\tau,j}}}
\\&=
\frac{e^{-\eta\sum_{\tau=1}^t\ell_{\tau,i}}}{\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t\ell_{\tau,j}}}
\end{align}
Thus for simplicity we refer to $\tilde{\ell}$ as $\ell$ in the followings.

S

% \textbf{Proof} 
\subsection{Proof of Lemma 1}
Starting with a uniform distribution over the coordinates $w_{0,i}\equiv \frac{1}{D}$ such that $W_0 = 1$ and we have:
\begin{align}
    W_{t+1} &= \sum_{i\in \mathcal{I}} w_{t+1,i} \leq 
    \sum_{\mathcal{I}_t\in \mathcal{S}}\prod_{i\in\mathcal{I}_t}w_{t+1,i}
    \\&=
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}W_t^{-1}\prod_{i\in\mathcal{I}_t}w_{t,i}e^{-\eta\ell_{t,i}} 
    \\&\leq \label{eq:sum_leq_1}
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}W_t^{-|\mathcal{I}_t|}\prod_{i\in\mathcal{I}_t}w_{t,i}e^{-\eta\ell_{t,i}} \cdot|perm(\mathcal{I}_t)|
    \\&=
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\prod_{i\in\mathcal{I}_t}\frac{w_{t,i}}{W_t}e^{-\eta\ell_{t,i}}\cdot \sum_{p\in perm(\mathcal{I}_t)}1 
    \\&=
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\prod_{i\in\mathcal{I}_t}\pi_{t,i}e^{-\eta\ell_{t,i}}\cdot \sum_{p\in perm(\mathcal{I}_t)}\prod_{k\in p}1 
    \\&\leq 
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}e^{-\eta\sum_{i\in\mathcal{I}_t}\ell_{t,i}}\prod_{i\in\mathcal{I}_t}\pi_{t,i}\cdot\sum_{p\in perm(\mathcal{I}_t)}\prod_{k\in p}\left(1-\sum_{j\in p_{1:k}}\pi_{t,j}\right)^{-1}
    \\&= \label{eq:back_to_pi_hat}
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}e^{-\eta\sum_{i\in\mathcal{I}_t}\ell_{t,i}}
    \\&\leq 
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}e^{-\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}}
    \\&\leq \label{eq:exp_ineq}
    W_t\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\left(1-\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}+\eta^2\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2\right)
    \\&\leq \label{eq:pi_hat_sums_to_1}
    W_t|\mathcal{C}|\left(1+\sum_{\mathcal{I}_t\in \mathcal{S}}\frac{\eta^2}{|\mathcal{C}|}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{C}||\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)
    \\&\leq \label{eq:exp_ineq_2}
    W_t |\mathcal{C}|e^{\sum_{\mathcal{I}_t\in \mathcal{S}} \frac{\eta^2}{|\mathcal{C}|}\hat{\pi}_{t,\mathcal{I}_t}\hat{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{C}||\mathcal{I}_t|}\hat{\pi}_{t,\mathcal{I}_t}\hat{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i}} 
\end{align}
Where
\begin{itemize}
    \item (\ref{eq:sum_leq_1}) holds since $W_0=1$ and $W_t$ is monotonically non-increasing following the update rule (\ref{eq:multiplicative_weight_update}) with non-negative losses, thus $w_t\leq 1$ for all $t$.
    \item (\ref{eq:back_to_pi_hat}) follows from (\ref{eq:common_numerator}).
    \item (\ref{eq:exp_ineq}) holds since $e^x\leq 1-x+x^2$ for all $x\geq 0$.
    \item (\ref{eq:pi_hat_sums_to_1}) holds since $\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}=|\mathcal{C}|$.
    \item (\ref{eq:exp_ineq_2}) holds since $1+x\leq e^x$.
\end{itemize}

Given that the sum of weights of a certain coordinate block $C^*$ is less than the total sum of weights, together with Eq.~\ref{eq:exp_ineq_2}, $w_{0,i}\equiv\frac{1}{D}$ and $W_0=1$ we have:
\begin{align}
   \frac{1}{D}\sum_{i\in C^*}e^{-\eta\sum_{t=1}^T\ell_{t,i}}
   = \sum_{i\in C^*} w_{t,i} \leq W_T 
   \leq 
    |\mathcal{C}|^T e^{\sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}} \eta^2\hat{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\hat{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i}} 
\end{align}
Taking the $\log$ of both sides, we have:
\begin{align} \label{eq:recursive_ineq}
  \log&\left(\sum_{i\in C^*}e^{-\eta\sum_{t=1}^T\ell_{t,i}}\right) 
  -\log(D) 
  \notag \\ &\leq \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}} \eta^2\hat{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\hat{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i} 
  + T\log(|\mathcal{C}|)
\end{align}
Following the same certain block, all the participating coordinates suffer the same loss 
 $\ell^*_t$ at every time step as follows from Eq.~\ref{eq:alpha_beta_loss}, hence:
 \begin{align} \notag
     \log\left(\sum_{i\in C^*}e^{-\eta\sum_{t=1}^T\ell_{t,i}}\right)
     &=
     \log\left(\sum_{i\in C^*}e^{-\eta\sum_{t=1}^T\ell^*_t}\right)
     \\ & = \notag
     \log\left(|C^*|e^{-\eta\sum_{t=1}^T\ell^*_t}\right)
     \\&=  \notag
     \log(|C^*|) -\eta\sum_{t=1}^T\ell^*_t
     \\ &\geq \label{eq:common_loss_ineq}
     -\eta|\mathcal{C}|\sum_{t=1}^T\ell^*_t
 \end{align}
 Thus Eq.~\ref{eq:recursive_ineq} and \ref{eq:common_loss_ineq} yield:
 \begin{align}
     -\eta|\mathcal{C}|\sum_{t=1}^T\ell^*_t -|\mathcal{C}|\log(D) 
     \leq \sum_{t=1}^T\sum_{\mathcal{I}_t\in \mathcal{S}} \eta^2\hat{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\hat{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i}
     + T\log(|\mathcal{C}|)
 \end{align}
 And since $\sum_{\mathcal{I}_t\in\mathcal{S}}$ is equivalent to $\sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}$, we have:
 \begin{align}
    \sum_{t=1}^T\sum_{c\in\mathcal{C}}&\frac{1}{|\mathcal{C}|}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\hat{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} - \sum_{t=1}^T \ell^*_t
    \notag \\ & \leq 
    \eta \sum_{t=1}^T\sum_{c\in\mathcal{C}}\frac{1}{|\mathcal{C}|}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\hat{\pi}_{t,\mathcal{I}_t}\cdot \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 + \frac{\log(D)}{\eta} 
    + T\frac{\log(|\mathcal{C})|}{|\mathcal{C}|}
 \end{align}
 
 
%  \textbf{Theorem 1}  Apply the update rule in \ref{eq:multiplicative_weight_update}, with a modified $\eta=\log(\alpha\beta)^{-1}\sqrt{\frac{\log(D)}{T}}$, then:
%  \begin{equation*}
%      Regret_t = \mathcal{O}(\log(\alpha\beta)\sqrt{T\log(D)})
%  \end{equation*}
 
%  \textbf{Proof} 
\subsection{Proof of Theorem 1}
 Since $\ell_{t,i} \leq \log(\tilde{\alpha}\tilde{\beta})$ then: 
 \begin{align}
     \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2
     \leq
     \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\log(\tilde{\alpha}\tilde{\beta})\right)^2
     \leq
     \log(\tilde{\alpha}\tilde{\beta})^2
 \end{align}
 
 Thus since $\sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}=|\mathcal{C}|$ we have,
 \begin{align}
     \sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\cdot \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2
     \leq
     \sum_{\mathcal{I}_t\in \mathcal{S}}\hat{\pi}_{t,\mathcal{I}_t}\log(\tilde{\alpha}\tilde{\beta})^2
     =
     |\mathcal{C}|\log(\tilde{\alpha}\tilde{\beta})^2
 \end{align}
 And Eq.~\ref{eq:lemma_1} yields,
 \begin{equation}
     Regret_t \leq \eta T \log(\tilde{\alpha}\tilde{\beta})^2 
     + \frac{\log(D)}{\eta}
     + T\frac{\log(|\mathcal{C}|)}{|\mathcal{C}|}
     = 2 \log(\tilde{\alpha}\tilde{\beta})\sqrt{T\log(D)}
 \end{equation}

==> regret/regret_combinatorial_backup.tex <==
\subsection{Regret analysis for sampling from the combinatorial space of coordinate blocks} \label{sec:comb_regret_analysis}
In this section we provide proofs for the theorems in Sec.~\ref{ss:analysis}.

The probability $\tilde{\pi}_{t,\mathcal{I}_t}$ of selecting a certain coordinate block $\mathcal{I}_t\subset \mathcal{I}=\{1,\cdots,D\}$ of size $|\mathcal{I}_t|=c\in\mathcal{C}$ follows sampling according to $\pi_t$ such that: 
\begin{align}\label{eq:block_prob}
    \tilde{w}_{t,\mathcal{I}_t} = 
    \prod_{i\in \mathcal{I}_t}w_{t,i}^{\frac{1}{|\mathcal{I}_t|}}
    \quad ; \quad
    \tilde{W}_t = \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\tilde{w}_{t,\mathcal{I}_t}
    \quad ; \quad
    \tilde{\pi}_{t,\mathcal{I}_t} = \frac{\tilde{w}_{t,\mathcal{I}_t}}{\tilde{W}_t}
    \quad \forall \mathcal{I}_t \in \bigcup_{c\in\mathcal{C}}\mathcal{S}_c
\end{align}
such that 
\begin{equation} \label{eq:prob_sum_to_1_2}
    \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\tilde{\pi}_{t,\mathcal{I}_t} =1
\end{equation}

In addition, let us first modify the losses in Eq.~\ref{eq:alpha_beta_loss} to be non-negative by adding the same constant $\log(\alpha)$ to all possible values:
\begin{align} \label{eq:alpha_beta_loss_shifted}
    \tilde{\ell}_{t,i} =
    \begin{cases}
		0 & \text{if } i \in C_t \text{ and } y_t > M_{t-1} \\
		\log(\tilde{\alpha}\tilde{\beta}) & \text{if } i \in C_t \text{ and } y_t \leq M_{t-1} \\
        \log(\tilde{\alpha}) & \text{if } i \notin C_t
    \end{cases}
\end{align}
This modification does not change the resulted distribution $\pi_t$ induced over the coordinates as it is invariant to shifts of the losses:
\begin{align}
\notag
\pi_{t,i} = \frac{w_{t,i}}{W_t} &= \frac{e^{-\eta\sum_{\tau=1}^t\tilde{\ell}_{\tau,i}}}{\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t\tilde{\ell}_{\tau,j}}} =
\frac{e^{-\eta\sum_{\tau=1}^t(\ell_{\tau,i}+\log(\tilde{\alpha}))}}{\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t(\ell_{\tau,j}+\log(\tilde{\alpha}))}}
=
\frac{e^{-\eta t\log(\tilde{\alpha})}e^{-\eta\sum_{\tau=1}^t\ell_{\tau,i}}}{e^{-\eta t\log(\tilde{\alpha})}\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t\ell_{\tau,j}}}
\\&=
\frac{e^{-\eta\sum_{\tau=1}^t\ell_{\tau,i}}}{\sum_{j=1}^D e^{-\eta\sum_{\tau=1}^t\ell_{\tau,j}}}
\end{align}
Thus $\tilde{\pi_{t,i}}$ remains unchanged as well and for simplicity we refer to $\tilde{\ell}$ as $\ell$ in the followings.

% \textbf{Proof} 
\subsubsection{Proof of Lemma 1}
\textbf{Lemma 1} For $\eta >0$ and non-negative losses $\ell_{t,i}\geq 0$ the update rule in (\ref{eq:multiplicative_weight_update}) satisfies for any block of coordinates $C^*$:
\begin{equation}\label{eq:lemma_1_2}
 \sum_{t=1}^T\sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in \mathcal{S}_c}\tilde{\pi}_{t,\mathcal{I}_t}\cdot\frac{1}{|\mathcal{I}_t|} \sum_{i\in\mathcal{I}_t}\ell_{t,i} 
 -\sum_{t=1}^T\frac{1}{|C^*|}\sum_{i\in C^*}\ell_{t,i}
\leq 
\eta\sum_{t=1}^T\sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in \mathcal{S}_c}\tilde{\pi}_{t,\mathcal{I}_t}\cdot \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 + \frac{D\log(D)}{\eta}
\end{equation}

\textbf{Proof}: Set: 
\begin{equation} \label{eq:init_2}
    \tilde{w}_{0,\mathcal{I}_t} = 1 \quad \forall \mathcal{I}_t \in \bigcup_{c\in\mathcal{C}}\mathcal{S}_c
\end{equation}
Thus,
\begin{align}
    \tilde{W}_{t+1} &= 
    \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\tilde{w}_{t+1,\mathcal{I}_t}
    =
    \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\prod_{i\in \mathcal{I}_t}w_{t+1,i}^{\frac{1}{|\mathcal{I}_t|}}
    \\ & =
    \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\prod_{i\in \mathcal{I}_t}w_{t,i}^{\frac{1}{|\mathcal{I}_t|}}e^{-\frac{\eta}{|\mathcal{I}_t|}\ell_{t,i}}
    =
    \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\prod_{i\in \mathcal{I}_t}w_{t,i}^{\frac{1}{|\mathcal{I}_t|}}\cdot e^{-\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}}
    \\ & = 
    \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\tilde{w}_{t,\mathcal{I}_t}\cdot e^{-\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}}
    \\ & = \label{eq:back_to_pi_hat_2}
    \tilde{W}_t\sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\tilde{\pi}_{t,\mathcal{I}_t}\cdot e^{-\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}}
    \\&\leq \label{eq:exp_ineq_1_2}
    \tilde{W}_t\sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in \mathcal{S}_c}\tilde{\pi}_{t,\mathcal{I}_t}\left(1-\frac{\eta}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}+\eta^2\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2\right)
    \\&\leq \label{eq:pi_hat_sums_to_1_2}
    \tilde{W}_t\left(1+
    \sum_{c\in\mathcal{C}}\left(\sum_{\mathcal{I}_t\in \mathcal{S}_c} \eta^2\tilde{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\tilde{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)
    \right)
    \\&\leq \label{eq:exp_ineq_2_2}
    \tilde{W}_t e^{
    \sum_{c\in\mathcal{C}}\cdot\left(\sum_{\mathcal{I}_t\in \mathcal{S}_c} \eta^2\tilde{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\tilde{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)
    } 
\end{align}
Where,
\begin{itemize}
    \item (\ref{eq:back_to_pi_hat_2}) follows from (\ref{eq:block_prob}).
    \item (\ref{eq:exp_ineq_1_2}) holds since $e^{-x}\leq 1-x+x^2$ for $x\geq 0$.
    \item (\ref{eq:pi_hat_sums_to_1_2}) holds due to Eq.~\ref{eq:prob_sum_to_1_2}.
    \item (\ref{eq:exp_ineq_2_2}) holds since $1+x\leq e^x$.
\end{itemize}

Due to Eq.~\ref{eq:init_2} we have,
\begin{align} \label{eq:aggergate_block_losses}
  \tilde{w}_{t,\mathcal{I}_t} 
  = 
  \prod_{i\in \mathcal{I}_t}w_{t,i}^{\frac{1}{|\mathcal{I}_t|}} 
  =
  \prod_{i\in \mathcal{I}_t}w_{0,i}^{\frac{1}{|\mathcal{I}_t|}} e^{-\frac{\eta}{|\mathcal{I}_t|}\sum_{t=1}^T\ell_{t,i}}
  =  e^{-\frac{\eta}{\mathcal{I}_t}\sum_{t=1}^T\sum_{i\in \mathcal{I}_t}\ell_{t,i}}
\end{align}
And,
\begin{equation}\label{eq:big_init_2}
   W_0=\sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}\tilde{w}_{0,\mathcal{I}_t}
   =\sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in\mathcal{S}_c}1
   =\sum_{c\in\mathcal{C}}|\mathcal{S}_c|=
   \sum_{c\in\mathcal{C}}{D \choose c} \leq (D!)^{|\mathcal{C}|}
\end{equation}
Given that the weight of a certain coordinate block $C^*$ is less than the total sum of all weights, together with Eq.~\ref{eq:exp_ineq_2_2},~\ref{eq:init_2} and~\ref{eq:big_init_2} we have:
\begin{align}
   e^{-\frac{\eta}{|C^*|}\sum_{t=1}^T\sum_{i\in C^*}\ell_{t,i}}
   &=  
   \tilde{w}_{t,C^*} \leq \tilde{W}_T 
   \notag \\ &\leq 
   (D!)^{|\mathcal{C}|} e^{
   \sum_{t=1}^T\sum_{c\in\mathcal{C}}\cdot\left(\sum_{\mathcal{I}_t\in \mathcal{S}_c} \eta^2\tilde{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\tilde{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)
  } 
\end{align}
Taking the $\log$ of both sides, we have:
\begin{align} \label{eq:recursive_ineq_2}
-\eta\sum_{t=1}^T\frac{1}{|C^*|}\sum_{i\in C^*}\ell_{t,i}
  & \leq
  \sum_{t=1}^T\sum_{c\in\mathcal{C}}\cdot\left(\sum_{\mathcal{I}_t\in \mathcal{S}_c} \eta^2\tilde{\pi}_{t,\mathcal{I}_t}\left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2 -\frac{\eta}{|\mathcal{I}_t|}\tilde{\pi}_{t,\mathcal{I}_t}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right) 
%   \notag \\& 
  + |\mathcal{C}|\log(D!)
\end{align}
and since $D!\leq D^D$ 
% due to the Stirling approximation~\cite{pearson1924historical} for large $D$ 
the result follows.
 
  \textbf{Theorem 1}  Apply the update rule in \ref{eq:multiplicative_weight_update}, with a modified $\eta=\log(\alpha\beta)^{-1}\sqrt{\frac{\log(D)}{T}}$, then:
%  \begin{equation*}
%      Regret_t = \mathcal{O}(\log(\alpha\beta)\sqrt{T\log(D)})
%  \end{equation*}
 
\textbf{Proof}: Since $\ell_{t,i} \leq \log(\tilde{\alpha}\tilde{\beta})$ then: 
 \begin{align}
     \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2
     \leq
     \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\log(\tilde{\alpha}\tilde{\beta})\right)^2
     \leq
     \log(\tilde{\alpha}\tilde{\beta})^2
 \end{align}
 
 Thus due to Eq.~\ref{eq:prob_sum_to_1_2}:
 \begin{align}
    \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in \mathcal{S}_c}\tilde{\pi}_{t,\mathcal{I}_t}\cdot \left(\frac{1}{|\mathcal{I}_t|}\sum_{i\in\mathcal{I}_t}\ell_{t,i}\right)^2
     \leq
     \sum_{c\in\mathcal{C}}\sum_{\mathcal{I}_t\in \mathcal{S}_c}\tilde{\pi}_{t,\mathcal{I}_t}\log(\tilde{\alpha}\tilde{\beta})^2
     =
     \log(\tilde{\alpha}\tilde{\beta})^2
 \end{align}
 And setting $\eta=\frac{1}{\log(\tilde{\alpha}\tilde{\beta})}\sqrt{\frac{|\mathcal{C}|D\log(D)}{T}}$ in Eq.~\ref{eq:lemma_1_2} yields:
 \begin{equation}
     Regret_t \leq \eta T \log(\tilde{\alpha}\tilde{\beta})^2 + \frac{|\mathcal{C}|D\log(D)}{\eta}
    = 
     2 \log(\tilde{\alpha}\tilde{\beta})\sqrt{T|\mathcal{C}|D\log(D)}
 \end{equation}
